Unintended Memorization and Timing Attacks in Named Entity Recognition Models

Named entity recognition models (NER), are widely used for identifying named entities (e.g., individuals, locations, and other information) in text documents. Machine learning based NER models are increasingly being applied in privacy-sensitive applications that need automatic and scalable identification of sensitive information to redact text for data sharing. In this paper, we study the setting when NER models are available as a black-box service for identifying sensitive information in user documents and show that these models are vulnerable to membership inference on their training datasets. With updated pre-trained NER models from spaCy, we demonstrate two distinct membership attacks on these models. Our first attack capitalizes on unintended memorization in the NER's underlying neural network, a phenomenon NNs are known to be vulnerable to. Our second attack leverages a timing side-channel to target NER models that maintain vocabularies constructed from the training data. We show that different functional paths of words within the training dataset in contrast to words not previously seen have measurable differences in execution time. Revealing membership status of training samples has clear privacy implications, e.g., in text redaction, sensitive words or phrases to be found and removed, are at risk of being detected in the training dataset. Our experimental evaluation includes the redaction of both password and health data, presenting both security risks and privacy/regulatory issues. This is exacerbated by results that show memorization with only a single phrase. We achieved 70% AUC in our first attack on a text redaction use-case. We also show overwhelming success in the timing attack with 99.23% AUC. Finally we discuss potential mitigation approaches to realize the safe use of NER models in light of the privacy and security implications of membership inference attacks.

==> MI-text classification - PETS 2023/background.tex <==
\section{Background and Threat Model}\label{sec:background}
We first introduce background on neural networks and neural network based NER models before providing detailed implementation by spaCy's NER~\cite{entityrecognizer}. We then define our threat model and motivate our study. %\footnote{https://spacy.io/api/entityrecognizer} We then define our threat model and emphasize the motivation of our study on NER models. 
% 
% ~\cite{spacy}

\subsection{Neural Networks}
A Neural Network (NN) model seeks to learn a function $f_\theta$ through training data, where ${\theta}$ represents the parameters of the model~\cite{bengio2017deep}. 
%The training set $X = \{(x_i, y_i)\}_i^m$ consists of (multi-dimensional) data points $x_i$ together with their labels $y_i$. 
% The model is trained using an optimization function (e.g., gradient descent~\cite{qian1999momentum}) on a loss function (e.g., cross-entropy loss~\cite{zhang2018generalized}) that measures how well the model has learned the training data on a validation dataset. During training, the model is exposed to the training dataset in mini-batches,
% which correspondingly update the internal weights ${\theta}$, 
% the optimization function then updates these weights using a learning rate to optimize the function $f_\theta$. 
%is a function that learns the mapping between data points and labels . During the learning process, the model attempts to build a function $f_\theta$, where ${\theta}$ are the parameters of the function. The function $f_\theta$ not only learns from the provided training examples but also learns to generalize beyond the specific examples. In a traditional machine learning pipeline, a training set $X = \{(x_i, y_i)\}_i^m$ is passed to the model with $m$ pairs of data points ($x_i$) and class ($y_i$). The pairs are then parsed by the model to learn how data points ($x$) are mapped to each corresponding label ($y$). The model is trained using an optimization function (e.g., gradient descent~\cite{}) on a loss function (e.g., cross-entropy loss~\cite{}) that measures how well the model has learned the training data on a validation dataset. During training, the model is exposed to the training dataset in mini-batches,
% which correspondingly update the internal weights ${\theta}$, 
%the optimization function then updates these weights by adjusting the old weights using a learning rate $r$ to finally optimize the function $f_\theta$.
During training, data is passed over the model multiple times to learn $theta$ for high prediction accuracy. These iterations are relevant in the context of information leakage and memorization as some examples may be seen by the model multiple times despite only appearing once in the training set. This is a potential factor in the model memorizing data points as we shall demonstrate in Section~\ref{sec:MIA_memorization}.

\subsection{Neural Network based Named Entity Recognition} \label{nn_based_lm}
Named Entity Recognition (NER) is a natural language processing task that can automatically identify named entities in a text and classify them into predefined categories~\cite{nadeau2007survey}. The identified entities can then be used in downstream applications such as information retrieval, relation extraction, and de-identification~\cite{yadav2019survey,dernoncourt2017identification}.
Recently, neural network based NER systems have become popular and have achieved state-of-the-art performance~\cite{yadav2019survey, lample2016neural, ma2016end}. Various neural network architectures for NER have been proposed including feed-forward NN, Long-Short Term Memory (LSTM) network, bi-directional LSTM network~\cite{Chiu2016NamedER}, Convolutional Neural Network (CNN) or combination of these~\cite{Chiu2016NamedER, ge2020fedner}. 
%For instance, Lample et al.~\cite{lample2016neural} proposed two neural architectures for NER task:
% which rely on small amount of supervised training data and unlabeled corpora, 
%a bi-directional LSTM network with a sequential Conditional Random Fields (CRF) layer above it (LSTM-CRF) and a model based on transition-based parsing and stack LSTM (S-LSTM).
%Chiu et al.~\cite{Chiu2016NamedER} proposed a hybrid model of bi-directional LSTM and CNN for NER task. Specifically, words and characters are transformed into continuous vector representations, which are then concatenated and fed into the bi-directional LSTM network and then to the output layer for tagging named entities. The CNN is used to extract character features from each word. 
%Ge et al.~\cite{ge2020fedner} proposed a medical NER model that uses a combination of CNN and bi-directional LSTM over the word representations to learn dependency between words. The CNN layer captures the local text information whereas the bi-directional LSTM layer models long distance dependencies between words in both directions to capture global contexts. It then uses a CRF layer to decode word labels. This model incorporates three types of embedding to represent a word, i.e. pre-trained word embedding, a character embedding and a language model embedding.

Word embeddings are used in NN based NER models to transform a raw textual representation of the input space into a low-dimensional vector representation. Specifically, word embeddings are look-up tables that map each word from a vocabulary to a vector~\cite{song2020information}. Popular word embedding models include Word2Vec~\cite{bojanowski2017enriching}, GloVe~\cite{pennington2014glove} and FastText~\cite{mikolov2013distributed}. In addition, character-level embedding is also used to represent a word~\cite{ge2020fedner,Chiu2016NamedER}. Particularly, each character in a word is first assigned a character embedding of a fixed dimension. Embeddings of all characters in the words are given to a neural network such as a CNN which can learn the contextual representation of each character and output a character-level embedding of the given word. The character-level embedding is usually concatenated with the word-level embedding to form a word representation to be fed into the neural network. 

% In NN based language models,  raw textual representation of the input space, which is both discrete and sparse, is first transformed into a lower dimension vector representation. One such approach is the use of a text corpus, with a vocabulary, to be passed to an embedding model that transforms each word into its vector representation.
% %$v_w \in \mathbf{R}^d$ where $d$ is the dimension of the embedding (a hyper-parameter of the model), 
% Popular word embedding models include Word2Vec~\cite{bojanowski2017enriching}, GloVe~\cite{pennington2014glove} and FastText~\cite{mikolov2013distributed}. 

%Language models are statistical models that assign probabilities to words based on the context surrounding the word. 

%In this language learning task, the input space of text is both discrete and sparse, as a remedy, the traditional approach is to transform the raw textual representation of the input space into a lower dimension vector representation. One such approach is the use of a text corpus, with a vocabulary, to be passed to an embedding model that transforms each word into its vector representation.
%$v_w \in \mathbf{R}^d$ where $d$ is the dimension of the embedding (a hyper-parameter of the model), 
%Popular embedding models include Word2Vec~\cite{bojanowski2017enriching}, GloVe~\cite{pennington2014glove} and FastText~\cite{mikolov2013distributed}.

% \hassan{Include reference to some standard textbook, so interested reader can go into details. Also, to save symbols to use for later notations, if it is not needed, we do not have to include mathematical description above. E.g., use of $V$ and $E$ and $v_w$.}

% The use of word embeddings in a language model is often the first transformative step, its result is then used by subsequent stages of the model architecture. Often pre-trained word embedding models are used to enhance the transformation of unlabeled corpus. These pre-trained generic models learn the embedding function from a substantially larger corpus, for the general task of understanding language, from which the embedding can learn a new to the subsequent task (e.g. NER~\cite{Chiu2016NamedER})~\cite{song2020information}. %\hassan{Again reference this}


% The training data given to (re-)train the NER model is a collection of documents. Each document 
% is annotated as a sequence of words $x = (w_1, w_2, \ldots, w_n)$, together with one or more tuples of the form $(i, j, l)$, where $1 \le i \le j \le n$ are indexes and $l$ is a label (named entity) from a pre-defined set of labels $\mathcal{L}$. The tuple $(i, j, l)$ indicates that the subsequence of words $(w_i, \ldots, w_j)$ defines the entity $l$. %\tham{move to next section}

% After this, \emph{sentence embeddings} are used to map the sequence of tokens into a single embedding vector $f_\theta(x) \in \mathbb{R}^m$ by passing it to a neural network  $f_\theta$ to first transform the tokens into individual vectors $\mathbf{X} = (\mathbf{v}_1, \mathbf{v}_2, \ldots , \mathbf{v}_n)$. The vectors are then fed into another neural network (e.g., RNN, LSTM, Bi-LSTM, Tranformers) to obtain another representation $h = (\mathbf{h}_1, \mathbf{h}_2, \mathbf{h}_3, \ldots , \mathbf{h}_n)$ which carries sequential information about the tokens while reducing the representation to a single vector $f_\theta(x) \in \mathbb{R}^m$.
% \hassan{Please revisit: this is not really clear to me. A reference is also required}\tham{It seems the above text meant to described sentence embedding in general. I think we don't need to include it.}
%Specifically for NLP tasks, sentence embeddings are used to map a sequence of tokens $x = [w_1, w_2, w_3, ... , w_l]$ which are extracted during the tokenization of the input text of words, into a single embedding vector $f_\theta(x) \in \mathbf{R}$ by passing it to a neural network $f_\theta$ to first transform the tokens into individual vectors $\mathbf{X} = [v_1, v_2, v_3, ... , v_l]$. The vectors are then fed into another neural network (e.g., RNN, LSTM, Bi-LSTM, Tranformers) to obtain a hidden representation $h = [h_1, h_2, h_3, ... , h_l]$ for each token in $x$, while reducing the representation to a single vector $f_\theta(x) \in \mathbf{R}$. 
%\hassan{What is the difference between a word and a token? Also, what's the use of the ``hidden'' representation?}
% This representation holds contextual information in the sequence of word tokens of $x$, useful for applications such as token tagging~\cite{Chiu2016NamedER,lample2016neural} where the input to the model is a sequence of words $x$ and the output $y = (y_1,y_2, \ldots, y_n)$ is a sequence of scores assigned to each token in $x$. 

\begin{example}
Consider the sentence ``John Doe lives in the United States,'' given as input to a trained NER model. An example (simplified) output of the model looks like: 
\begin{quote}
    ``John Doe [PERSON, score] lives [O, score] in [O, score] the [O, score] United States [LOCATION, score].'' 
\end{quote}
Here PERSON, LOCATION and O are pre-defined labels, where O stands for ``OUT,'' i.e., a label not in the set $L$ of pre-defined labels. The label assigned is the one with the highest probability score, a real number between 0 and 1 indicated above as ``score.'' The name John Doe is a multi-token entity, i.e., John is the first word in the entity indicated by the prefix ``B'' while Doe is the last, indicated by the prefix ``L'' (these prefixes are not shown in the above example). NER systems use tagging schemes such as the BILOU (Begin Inside Last Outside Unigram). For a document redaction application, we might then want to remove all instances of the entity PERSON. 
%For example, given an input sequence ``Donald Trump lives in the United States'', each word would be assigned a probability vector of size $k$ where each probability score refers to a tag. The name ``Donald Trump'' is a continuous entity, that is that the word Donald is the first word in the entity and is assigned the B-NAME tag while ``Trump'' being the last and gets assigned the L-NAME tag. NER systems use tagging schemes such as the BILOU (Begin Inside Last Outside Unigram) tagging scheme. 
\end{example}


% \hassan{It will be helpful to give a toy example here with actual words}

%In a majority of NLP tasks, the input to the NLP model is a variable length sequence of words/tokens within the embedding space. The output can be a class label (e.g., text classification, sentiment analysis), a word/token (e.g., predictive models for next word prediction) or another variable length sequence of words/tokens (e.g., machine translation). 

%In this paper, we study the privacy of the named entity recognition (NER) model which takes a sequence of words as input and returns predefined tags/labels to some words that are identified as named entities. 
%For example,   
% In this paper we experiment with spaCy's Named Entity Recognition (NER) component, functionally a system that assigns tags to each word in a text input of a variable length. 
%Each word is assigned a label based on the probability scores which is also seen in the model's output.
%For example, given the input text ``Donald Trump lives in the United States'' to the NER model, the output is a sequence of named entities assigned to words, i.e., ``Donald Trump [PERSON, 'score'] lives [O, 'score' ] in [O, 'score'] the [O, 'score'] United States [LOCATION, 'score']''. \tham{@Rana can you please confirm the probability score for each label in the output?}
%\hassan{Is this the same as assigning a class label? This example does not appear above. Also, since this is our use-case, we need to be more precise here, and explain what does the output look like, i.e., probability vector of labels?.}

% \subsection{Named Entity Recognition}
% \hassan{I recommend condensing this and merging this with the previous section, and calling the section Neural Network based Named Entity Recognition}

% Named Entity Recognition (NER) is known as a natural language processing task that can automatically identify named entities in a text and classify them into predefined categories~\cite{nadeau2007survey}. The identified entities can then be used in downstream applications such as information retrieval, relation extraction, de-identification~\cite{yadav2019survey}.
% Traditional method used in early NER systems is based on handcrafted rules which requires domain experts for constructing the rules. 
% Supervised machine learning algorithms including Hidden Markov Model, Support Vector Machines, Conditional Random Fields and Decision Trees are also widely used for NER task~\cite{florian2003named, krishnan-manning-2006-effective} which takes human labelled documents as training data. However, they requires large collection of annotated data corpus which remain limited in specific domains and languages.

% It is a complex task requiring structured training data from which to learn from, a resource that is not widely available. 
% This lack of training examples leads to NER models not generalizing to the extent of a model with significantly more data. 

% Recently, neural network based NER systems have become popular and achieved the state-of-the-art performance~\cite{yadav2019survey, lample2016neural, ma2016end}. Various neural network architectures for NER have been proposed including feed-forward NN, Long-Short Term Memory (LSTM) network, bi-directional LSTM network, Convolutional Neural Network (CNN) or combination of these. 
% The neural networks learn important features from word embeddings and/or character embeddings.
% Collobert et al.,~\cite{collobert2011natural} proposed a model using a CNN over a sequence of word embeddings to capture the context and a Conditional Random Fields (CRF) layer on top of the CNN. 
% Chiu et al.,~\cite{Chiu2016NamedER} proposed NER model using a hybrid bi-directional long-short term memory (BLSTM) network and CNN architecture. Specifically, words and characters are transformed into continuous vector representations, which are then concatenated and fed into the BLSTM. In addition, a CNN is used to induce character-level features. Recently, Lample et al.,~\cite{lample2016neural} proposed two neural architectures for NER task which rely on small amount of supervised training data and unlabeled corpora, a bi-directional LSTM network with a sequential CRF layer above it (LSTM-CRF) and a model based on transition-based parsing and stack LSTM (S-LSTM). 
% Ge et al.,\cite{ge2020fedner} proposed a medical NER model that uses a combination of CNN and bi-directional LSTM over the word presentations to learn dependency between words. The CNN layer captures the local text information whereas the bi-directional LSTM layer models long distance dependencies between words in both directions to capture global contexts. It then uses the CRF to decode word labels. In this work, a pre-trained word embedding, a character embedding and a language model embedding are concatenated to represent a word.   

% \tham{work in progress}

% The NER model implemented in spaCy library based on a CNN over word embeddings and transition-based dependency parsing. In the following section, we describe the NER model implemented in spaCy library in details.

\subsection{spaCy's NER model}
\label{ner_spacy}
% Named Entity Recognition is a complex task requiring structured training data from which to learn from, a resource that is not widely available. This lack of training examples leads to NER models not generalizing to the extent of a model with significantly more data.

% \textbf{SpaCy's NER model: Transition-based NER}
% To address this limitation, 
% spaCy's NER implementation is constructed using a multi-layer model that first leverages well generalized word embeddings to create a context-based sentence embedding (the context is sourced from word embeddings surrounding the target word). Architecturally, the NER model includes a deep CNN and a transition-based parser using chunking models as defined in~\cite{lample2016neural}. \hassan{What are chunking mdoels?}

spaCy\footnote{Unless otherwise specified we refer to spaCy Version 3.0.3} builds a transition-based parser which can apply to both NER and dependency parsing tasks. The transition-based parsing is an approach to structured prediction where the task of predicting the structure is mapped to a series of state transitions~\cite{lample2016neural, kuhlmann-etal-2011-dynamic}. The underlying neural network state prediction model consists of either two or three
subnetworks: \textit{tok2vec}, \textit{lower} and \textit{upper} (optional). The \textit{tok2vec} subnet uses hash embedding with sub-word features and a CNN with layer-normalized maxout to map each word into a vector representation. The \textit{lower} subnet constructs a feature-specific vector for each (token, feature) pair. The state representation is constructed by summing the component features and applying the non-linearity. The \textit{upper} subnet is an optional feed-forward network that predicts the action scores from the state representation. If it is not present, the output from the \textit{lower} subnet is used as action scores directly~\cite{spacyparser}.
%\footnote{https://github.com/explosion/spaCy/blob/master/spacy/ml/models/parser.py}

% Words embeddings are computed from unique multi-hash embeddings, which despite having a large vocabulary can uniquely identity word vectors using a size-restricted embedding table. In a normal embedding table, each word is mapped to its own vector; however in a hashed-embedded table, the words are first mapped to an arbitrary integer value by using the modulus remainder within the range of the length of the embedding table. 
% To obtain an index key to the embedding table, words are hashed with two different seeds to obtain two different keys. These two keys and corresponding vectors are the unique representation for a given word in the embedding table. This approach permits the use of a small embedding table, but still allows words to be assigned unique vectors.


% \hassan{The features come up again and again in the following sections. I think we should define these in more details, e.g., the shape, and the norm. Also, discuss the curious thing about the shape as two words of different length may have the same shape}
Four important features of the word are used to form its representation, which we call \emph{sub-word features}: \emph{norm}, \emph{prefix}, \emph{suffix} and \emph{shape}. The norm feature defines a normalised form of the word, i.e., normalising words with different spellings to one common spelling. At the very least, the norm contains a subsequence of the lower case form of the word. The prefix feature is defined as the first $n$ characters of the word where default value of $n$ is 1. The suffix feature is defined as the last $m$ characters of the word with default value of $m$ being 3. Both prefix and suffix are case-sensitive. The `shape' forms the orthographic feature of the word where lower-case, upper-case alphabetic characters and numeric characters are replaced by `x', `X' and `d' respectively, and special symbols are kept intact. It is noted that sequences of the same character shape (X, x or d) are truncated after length 4. Therefore, two words with different length may end up with the same shape. For example, two words \textit{Threats} and \textit{Embed} have the same shape of `Xxxxx'. The interested reader can refer to Appendix~\ref{app:equiv-proof}, to see 
%In the full version of this paper, we show 
when two words having the same set of features may in fact be different.

Figure~\ref{fig:spacy_ner_model} illustrates the architecture of the NER model in spaCy in detail. As visualized in the shaded green area in Figure~\ref{fig:spacy_ner_model}, the \textit{tok2vec} subnet first separately embeds the norm, prefix, suffix, and shape features of each word using hash embeddings. Each feature is assigned a unique vector. Then, vector representations of all features are concatenated together to get a word vector, ${e}_i = [e_i^{\text{prefix}}|e_i^{\text{suffix}}|e_i^{\text{norm}}|e_i^{\text{shape}}]$. 
If pre-trained vector table including pre-trained word embeddings is available, a static vector of the given word is also concatenated to the  word vector. The concatenated word vector is then passed to a \textit{max-out} layer to capture a context independent representation of each word. If there are $n$ words (tokens) in the input text as $(w_1, w_2,\ldots , w_n)$, then they are converted into $n$ embeddings as $(e_1, e_2, \ldots , e_n)$. 
%If there are $n$ tokens in the input text as $(w_1, w_2,\ldots , w_n)$, then they are converted into $n$ embeddings as $(e_1, e_2, \ldots , e_n)$. 
% In the multi-hash embedding architecture, spaCy takes four different features of a given word including the prefix (e.g., first character), suffix (e.g., last 3 characters), shape (e.g., '123qweR' $\rightarrow$ 'dddxxxX') and norm (e.g., lower form of a word). Each feature gets a distinct vector representation ${e}_i = [e_i^{\text{prefix}}|e_i^{\text{suffix}}|e_i^{\text{norm}}|e_i^{\text{shape}}]$ using the hashing technique, which is then concatenated with vector representations of other features. The concatenated vector is then passed to a \textit{max-out} layer to capture a context independent representation of each word. If there are $n$ tokens in the input text as $(w_1, w_2,\ldots , w_n)$, then they are converted into $n$ embeddings as $(e_1, e_2, \ldots , e_n)$. 
% spaCy also uses pre-trained word embeddings in the embedding layer so an additional feature of a word could also be used to compute the word level representation \hassan{<-- not clear what this means}. However, all out-of-vocabulary words are assigned the same vectors from the pretrained word embedding table.\hassan{<-- not clear what this means} 
In the next step in the \textit{tok2vec}, as illustrated in the shaded blue area in Figure~\ref{fig:spacy_ner_model}, the context independent vector representation $e_i$ of each word $w_i$ is passed to the encoding layer which consists of a CNN model, that takes a \emph{window size} as a hyperparameter. Through the window size, which by default is 1, spaCy captures the context around the given word. For instance, a window size of 1 captures the context of one word in each direction (i.e., $e_{i-1}, e_{i+1}$). Depending on the depth of the CNN (the number of convolutional layers), which is by default 3, the layer assigns a context dependent vector to each token in the text as $(c_1, c_2, c_3, \ldots , c_n)$. The receptive field of the CNN is defined as $\text{depth} \times ( \text{window-size} \times 2 + 1 )$.
% \[\text{depth} \times ( \text{window-size} \times 2 + 1 ).
% \]
%$depth$ $\times$ ($window$\textunderscore$size$ $\times$ 2 + 1).
With $\text{depth} = 3$, and $\text{window-size} = 1$, the network would be sensitive to 9 words at a time.

% The NER model architecture in the spaCy library is shown in  Figure~\ref{fig:spacy_ner_model}.



\begin{figure}
\includegraphics[width=\linewidth]{plots/Spacy-Model-Page-2.pdf}\label{fig:spacy}
\caption{SpaCy's NER Model. An input sentence is broken up into words which are individually processed into an embedding (shaded green). This embedding is then converted into a contextual Encoding, by combining the current word embedding with the embeddings of surrounding sentence words (shaded blue), before being processed by the Multi-Layer Perceptron.}
\label{fig:spacy_ner_model}
% \vspace{-6mm}
\end{figure}


For assigning labels to tokens, the NER model is based on a transition based parser which was inspired by the arc-standard parser~\cite{nivre2004incrementality}. As in NER tasks neighboring labels have some sort of relation with each other, a transition based approach takes into consideration the learned embedding of the label type from previously identified labels and uses that for the next prediction. With this approach the word that was assigned a label even far back in the document would also be considered when making a prediction for the current word~\cite{lample2016neural}.
%\tham{todo: Need to describe the \textit{lower} subnet in more details for how the prediction works} 
 

The training data given to (re-)train the spaCy NER model is a collection of documents. Each document 
is annotated as a sequence of words $x = (w_1, w_2, \ldots, w_n)$, together with one or more tuples of the form $(i, j, l)$, where $1 \le i \le j \le n$ are indexes and $l$ is a label (named entity) from a pre-defined set of labels $\mathcal{L}$. The tuple $(i, j, l)$ indicates that the subsequence of words $(w_i, \ldots, w_j)$ defines the entity $l$. The pre-trained NER model in spaCy includes 18 labels for pre-defined  named entities and uses BILOU tagging system. %, as defined earlier.. %https://github.com/explosion/spaCy/blob/master/spacy/pipeline/ner.pyx
A list of transition names are defined based on the pre-defined named entities and the tagging system, i.e. number of transition moves in spaCy NER is $18 \times 4 + 1 = 73.$

==> MI-text classification - PETS 2023/conclusion.tex <==
% \vspace{-3mm}
% \vfill
\section{Conclusion}\label{sec:conclusion}
Many emerging applications of Named Entity Recognition (NER) models show their potential to be monetized as a service, including identification of medical and other personal information in documents to minimise impacts of data breaches, and redaction of sensitive information for document sharing. With the spaCy NER model as a use case, we have shown that the current crop of neural network based NER models are vulnerable to privacy attacks on their underlying training data, and thus in their current form they are not suitable to be hosted as an online service for labeling sensitive information. We have demonstrated two main attacks on NER models, one based on neural network memorisation, and the other based on timing differences when queried with text appearing in the training dataset versus text outside the training dataset. Both attacks can be somewhat mitigated by using techniques such as differential privacy and timing delays, with obvious accuracy and efficiency tradeoffs. We hope our work motivates the pursuit for more privacy-preserving NER models.

==> MI-text classification - PETS 2023/defences.tex <==
\section{Possible Defences}\label{sec:defences}

\descr{Neural Memorization.} 
Memorizing training data poses serious privacy risk in machine learning. It is crucial to measure how much memorization occurs and propose solutions to mitigate this issue or at least to train the model with less memorization. 
Several possible approaches to mitigate unintended memorization of NNs in text generation were discussed in~\cite{carlini2019secret}. Among them, using differential privacy is demonstrated to be effective as it could fully eliminate unintended memorization in text predictive models~\cite[Sec 9.3]{carlini2019secret}. %\hassan{Anything specific to our use case? Can we enforce differential privacy in a way that if the example only occurs in the training document once, we do not use it to update the named entity?}
An emergent relationship between the number of unique documents in an entity class and the success of the membership inference attack was observed in Section~\ref{subsec:MIA_medical_dataset}. From this relationship, a simple means to reducing (but not eliminating) the success of a membership inference attack is to either eliminate the entity, likely an infeasible option as the capability to redact these infrequent entities is destroyed. Or alternatively, to generate, or source additional similar entities to train the model, to populate and reduce the risk posed by the under-represented entity class.
An approach to mitigate the proposed attack exploiting model's memorization demonstrated in Section~\ref{subsec:MIA_medical_dataset} is to restrict the NER model to return only the label of the queried text instead of without the confidence scores. Though we note that Label-only MI attacks have since been developed~\cite{li2020label,choo2020label}, we leave the evaluation of these label-only attacks as future work.

\descr{Timing Attack.} 
A possible defence to this vulnerability is to disable the updating vocabulary step during model training (or updating) so that sensitive words included in the private dataset are not added to the vocabulary. It is also noted that adding every unseen word's features to the vocabulary might make the model hosted in a cloud to be vulnerable to attacks which query the model with drivel, i.e., inundating the vocabulary with bogus words which could lead to space issues.  
 
Masking timing characteristics has been proposed to prevent against timing attacks in cryptosystems~\cite{kocher2018timing}. It is possible to apply this idea to prevent timing side-channel in NER models. {For instance, one} approach to mitigate the timing side-channel attack is to delay returning the result until a pre-defined time has elapsed. This would remove any timing difference, but impacts overall system speed. {Another approach specific to our scenario is to add a constant delay to the time of the member words.} For instance, on the updated LG NER model (cf. Section~\ref{timing_attack_updated_ner}), the average execution time taken by the model to process the member words and non-member words are $t_{\text{m}} = 2.08 \text{ms}$ and $t_{\text{nm}} = 2.44 \text{ms}$, respectively. {Assuming both time distributions to be normally distributed with means $t_{\text{m}}$ and $t_{\text{nm}}$, and the same variance, adding a time of $t_\text{nm} - t_\text{m}$ to the time of member words will make the two distributions identical, and hence thwart the timing attack. In practice system delays, or contested resources may result in a few outliers, in which case a trimmed mean can be employed. We note that the success of this defense can only be empirically determined as it relies on the accuracy of estimated mean times of member and non-member words, how accurately the distribution of times can be approximated as normally distributed, and the threshold to determine outliers. 
} 

{
\paragraph{Experiments:} In order to test the constant delay defense, we added the constant time of $t_\text{nm} - t_\text{m}$ to member queries in the experiments of Section~\ref{timing_attack_updated_ner}. To remove outliers, the we calculated a 10\% trimmed mean. For instance, a $t_\text{nm} - t_\text{m}= 36 \text{ms}$ delay is applied to the updated LG NER model. From Figure~\ref{fig:timing_sid_channel_def}, it is immediately evident that the timing attack can be thwarted with the addition of constant time. In all experimental settings, the MI AUC is close to 0.5, or a random guess.  The slight deviation from 0.5 is due to the fact that the timing distribution is not exactly standard normal (see Figure~\ref{fig:absolute_time_ner} in Appendix~\ref{sec:app:timing}). Compare this to Figure~\ref{fig:timing_sid_channel}, which depicts the MI ROC with no defense, where AUCs are close to 1.0. 
}

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{plots/timing_attack_auc_def.pdf}
% \vspace{-2mm}
\caption{{Constant time delay added to member words to defend against the timing side-channel attack. ROC curve classifies membership of word inputs.}
}
\label{fig:timing_sid_channel_def}
% \vspace{-3mm}
\end{figure}


%\hassan{The following to be removed. It does not necessarily prevent timing attack altogether. Instead we can add a constant delay of $t_\text{nm} - t_\text{m}$ to the time of in-vocab words. Assuming both member and non-member times are normally distributed with the same variance (reasonable assumption), this will make any distinguisher unsuccessful (the resulting distributions are equal)}.
%****************
%For instance, we can randomly add a delay during the processing of the model so that the model's execution time for processing member words and non-member words are less distinguishable. This can reduce the accuracy of the attack. 
%Consider a timing attack on the updated LG NER model (cf. Section~\ref{timing_attack_updated_ner}) the average execution time taken by the model to process the member words and non-member words are $t_{\text{m}} = 2.08 \text{ms}$ and $t_{\text{nm}} = 2.44 \text{ms}$, respectively. 
%We can simply sample a random delay from a uniform distribution with parameters $(t_{\text{nm}} - t_{\text{m}}, t_{\text{nm}})$ and add this delay during the processing of the model. By doing so, we can reduce the AUC of this attack from 0.994 to 0.649.  
%*****************
%Another approach to mitigate the timing side-channel attack is to delay returning the result until a pre-defined time has elapsed. This would remove any timing difference, but impacts overall system speed. 

\descr{Using Synthetic Data.} A potential defense to thwart MI attempts on either attack is replacing sensitive information in the private dataset with dummy information. However, this is not straightforward, as the owner will need to ensure that the dummy information at least preserves the semantics of the original information without degrading the accuracy of the NER model, e.g., length of ZIP codes, format of locations, and IP addresses, albeit in some cases, e.g., passwords, this may be possible. Moreover, this can be a tedious task for a large dataset, and some sensitive information may inadvertently be missed. Our attacks highlight the dangers of using sensitive datasets for training NER models without necessary protections. 
{
\paragraph{Experiments:} To test this mitigation measure we perform additional experiments with the i2b2 dataset. The i2b2 dataset is prepared by creating sets of members and non-members as in Section~\ref{subsubsec:i2b2_secret_redaction}. However, as an additional step, we replace instances of the sensitive label with dummy information from all training members. In particular, we choose the sensitive labels of Location and Contact, and replace all addresses and phone numbers with publicly available randomly generated synthetic ones.\footnote{\url{www.randomlists.com}} The model is then trained with this dummy training set. Note that the surrounding sentences remain the same. To test MIA accuracy we use the non-member set records from the same distribution as the original i2b2 dataset. We perform this experiment for two of the potentially vulnerable entities, i.e., Location and Contact. 

The results illustrated in Figure~\ref{fig:dummy_location} and \ref{fig:dummy_contact} show that the performance of the MI attack has now dropped to an AUC comparable to a random guess, demonstrating that a model trained with dummy data is less susceptible to membership inference attacks. This however, does result in a significant degradation of the model's ability to identify the correct entities due to the difference in the distribution of the dummy and original dataset. To resolve this trade-off, the task is to generate synthetic data such that the dummy data matches the original dataset's distribution, without compromising the privacy of the sensitive field. This means carefully crafting synthetic examples that capture sub-categories of the entities, e.g., the LOCATION category may contain different granularity of address information: from city, to zip code, to street address. This cannot be captured by simple data generation techniques such as the one used by us. We however leave this consideration for future work, given the setting and domain specificity of each sensitive entity. Figure~\ref{fig:defend_i2b2} in Appendix~\ref{app:full_docredact_loss}, shows the overall F1-score for all entities together with the standard deviation bands for these two experiments.}



\begin{figure}[t]
\centering
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.99\linewidth]{revised_plots/AUC_CONTACT-ORIGINAL_VS_DUMMY_i2b2_n2c2_dataset.pdf}
% \vspace{-3mm}
\caption{
{Original vs DUMMY LOCATION MI AUC}
}
\label{fig:dummy_location}
% \vspace{-5mm}
\end{subfigure}
%
\begin{subfigure}{\linewidth}
\centering
\includegraphics[width=0.99\linewidth]{revised_plots/AUC_LOCATION-ORIGINAL_VS_DUMMY_i2b2_n2c2_dataset.pdf}
% \vspace{-3mm}
\caption{
{Original vs DUMMY CONTACT MI AUC}
}
\label{fig:dummy_contact}
% \vspace{-5mm}
\end{subfigure}
\caption{{MI AUC comparison between Original dataset entity from Figure \ref{fig:i2b2_mia} vs DUMMY data for CONTACT and LOCATION.}}
% \vspace{-3mm}
\end{figure}

==> MI-text classification - PETS 2023/experiment.tex <==
\section{The Document Redaction Use-Case}
\label{sec:doc-redact}
We now turn to demonstrating our attack on a more practical use-case. We assume a service provider that builds on top of spaCy's NER model to provide an online document redaction service. The service provider uses a medical dataset containing sensitive information such as patient IDs, contact information and place of residence. The NER model is updated by training on this dataset to learn new labels specific to the application of medical data redaction. We call this the \emph{updating dataset}. These labels include ID, CONTACT and LOCATION. The updated NER model can then be queried via an API which customers can use to redact information within their documents. We assume an attacker who has access to the same API, and wishes to infer sensitive information (related to the labels) contained in the updating dataset. 

%\hassan{Two comments from reviewer are relevant to this section, for which I will write something:

%Impractical assumption. Also, the assumptions missed by the authors yet critical to the success of their approaches do not seem to be practical. For the first assumption, there is no justification that the formats of sensitive sentences in a dataset are all known. For the second assumption, it might be ok to consider ``Alice's secret is abcd'' as a member of victim's private dataset, since this helps reduce the searching space for the further attacks, but given the large number of similar secrets in one dataset, I doubt that the search space can be significantly reduced. Adding to the complexity is the relations between sensitive items, such as abc corresponding to Alice's secret not Bob's secret.

%Strange use-Case. In Section 4, the authors demonstrate a use-case on documents that contain user's ID, contact and location. However, they utilized an existing membership inference method [48] to accomplish the experiments, rather than the proposed method. There is no explanation about the relations between the known approach used for the attack and the proposed ones, which the authors may need to clarify.
%}

% To evaluate the exposure of a secret information in a text used to train the model we experimented based on multiple settings.
%In this section, we demonstrate that an adversary with a black-box access to an NER model can infer the membership information of sensitive words (medical ID of patients) in a medical dataset used to update the NER model. 

% \ben{Did we ever have results that described how good the NER models were? i.e. their Utility.} 
% \tham{We did discuss whether we need to report the performance of updated NER model, we thought it was not our concern. spaCy already reported ner's performance}
% \tham{The following was in the Use Case Section}


%\subsection{Document Redaction}
%Previously, the redaction of sensitive information from documents is a highly manual task requiring expertise and many hours to complete~\cite{gordon2013mra}. One of the major problems with redaction is that it can't be always content based, and for redacted information based on context more sophisticated process are required and as more documents are being generated, proposals have been made to automate document redaction to provide cost and time savings for the privacy-conscious document holder using text classification algorithms in natural language processing; However with the use of machine learning techniques for effective text classification, and subsequently text redaction may lead to privacy risks for the data used to train the models. To identify sensitive information, sensitive information would be used to train models, particularly if a model is to be tailored for a specific set of policies, a personalized process for each different company. As we demonstrate in our work, and as seen in previous works~\cite{kanchana2020optical, nivre2004incrementality}, dependency parser models like spaCy~\cite{honnibal2015improved} could be used to redact sensitive information from text. 

%Considering a setting where text classification models are used to classify and redact sensitive information from a given document~\cite{song2019auditing}. If an adversary has black-box access to the model and the redacted document used for training, the adversary could use the model's text classification feature to identify if some text was in the training data that was redacted. As we demonstrate in our work, and as seen in previous works~\cite{nivre2004incrementality}, dependency parser models like spaCy~\cite{honnibal2015improved} could be used to redact sensitive information from text. These models are trained on sensitive information to be classified as per need, the probability scores assigned to words per class could inadvertently leak information of the sensitive data used for training the models.

%We consider a similar setting where we use a data-set that contains patient medical documents~\cite{stubbs2015annotating} to update the NER model. Once the model is updated with such documents, it can be used to identify and redact sensitive information such as patient medical IDs, CONTACT information, LOCATION etc. \hassan{are we using surrounding text in this case? How do we know the surrounding text?} \ben{If I recall correctly, we query the original sentence this can vary from no prefix, to a sentence.}


% \subsection{Password Exposure}

%\subsection{Passwords, Credit Card Numbers, Phone Numbers, and IP addresses}


\subsection{The i2b2/UTHealth Corpus}
\label{subsec:MIA_medical_dataset}
We update the pre-trained spaCy NER model with the i2b2/UTHealth challenge dataset~\cite{stubbs2015annotating} which contains patient medical reports. These documents contain sensitive identifiers like names, IDs, contact, and location. We identify three sensitive labels (entities): ID, CONTACT and LOCATION for our experiments. We define a \emph{sample} for a label $l$ as any subsequence of words with the true label $l$ within these reports together with the surrounding sentence. We use the original training set (785 documents) and test set (511 documents) split from~\cite{stubbs2015annotating}. Samples from the training set are considered as members whereas those from the test set are non-members. Once again, we assume the attacker knows the surrounding sentences. Section~\ref{sub:unknown-surround} considers the case when the surrounding sentences may not be known by the attacker.

\descr{Attack Setup.} We use the membership inference attack proposed by Salem et al.~\cite{salem2019ml}, which uses the confidence score (probability score) returned by the model to infer membership. As mentioned before, the underlying assumption of this attack is that machine learning models may return a higher confidence score for training data points versus points seen by the model for the first time. In our case, the probability score is the score returned by spaCy when querying the model with a sample (of the three labels) from either the training or test dataset. We first train the model for 75 epochs with a batch size of 50 and evaluate the model's NER Test F1, and ROC Area Under the Curve (AUC) for membership inference after each epoch during training. Notice that since we have full training and test datasets, we can use the traditional AUC metric instead of the rank metric used in the previous section where we assessed membership inference of a single phrase.

\descr{Results.} Figure~\ref{fig:i2b2_mia} reports the AUC of the MI attack. Observe that there is a delay in the rise of the attack AUC for a few initial epochs due to the initial learning from the high number of samples for each entity in the training set. It is not until the test F1 score begins to plateau (training loss was also levelling off near 0) that we observe a sharp rise in the attack AUC above a random guess of 0.5. We also observe that the MI attack AUC for the ``LOCATION'' entity is higher than ``ID'' and ``CONTACT''. 
We hypothesize this is due to ``LOCATION'' words being linguistically common (and so the language model will contain knowledge of their semantics). This is also true, to a lesser extent of names in CONTACT entities. IDs, on the other hand is a string of numbers. Word embeddings are unlikely to include long numbers and thus unlikely to encode deeper semantics of numbers. However we note that the pre-trained NER model contains an existing ``LOCATION'' entity type. Contrary to our observation, one would expect a previously defined class in a pre-trained language model to already be sufficiently generalized to dissuade memorization. {The highest attack AUC is between 0.7 to 0.8, and even the lowest attack AUC is 0.6 (for the ID entity), well above the random guess mark of 0.5.} Therefore, we observe that MI succeeds in all cases. The relationship of MI accuracy between these entity classes is beyond the scope of this work.

% We hypothesis this is due to the complexity of data included within each entity, as ``LOCATION'' is featured in a relatively numerous 541 documents compared to a reduced 511 and 248 for ``ID'' and ``CONTACT'' observes a higher MI AUC. 

Above we observed that ``ID'' and ``CONTACT'' had less documents and MI AUC. But to ensure a lower number of documents representing these entities in the training set is not responsible for the decreased MI AUC, we withheld documents containing ``CONTACT'' samples. Curiously, we observed the opposite effect for the same complexity. Specifically we performed an attempt by taking only documents where the ``CONTACT'' word was longer than 5 characters (yielding 94 samples), we refer to this as ``CONTACT-5''. By further restricting this set to 50, 30 and 10 documents, we also obtain configurations of ``CONTACT-5-50'', ``CONTACT-5-30'', ``CONTACT-5-10'' respectively. We observe with a decreasing number of available samples representing an entity, the attack AUC increases. Therefore, the less documents for an entity, the more the model will memorize the entity. Note that the F1-score approaching one indicates that in all cases the model is not prone to overfitting after around 10 epochs. We note that the F1 curves for all datasets is approximately the same, and thus have been averaged in Figure~\ref{fig:i2b2_mia}. The individual F1-scores of each experiment together with the detailed standard deviation bands are included in Figure~\ref{fig:full_i2b2_loss} of Appendix~\ref{app:full_docredact_loss}.

%With the continued decrease in the number of available samples representing each entity class, the overall attack AUC is increased. From this we are able to conclude that the number of representative examples for each entity class is related to the memorization and this success of the MI attack.

%\hassan{What does it tell us? The less the number of samples for a given entity the more the likelihood of the model memorising? Also, any commentary on the Loss? It seems just by looking at the Loss we cannot tell if we have overtrained the model or not? It is not overfit in all cases.}
%\ben{comparing training and testing loss would be the method to detect overfitting. i.e. test loss goes back up at some point.}

% Figure~\ref{fig:i2b2_mia} reports the AUC of the MI attack. We infer that due to the high number of samples for each entity in the training set, the AUC doesn't increase after a few epochs. We also report AUC for the CONTACT entity to be higher than ID due to a lower number of samples in the training set.


\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]{revised_plots/AUC_CONTACT-ID-LOCATION-SECRET-30-50-100-150_i2b2_n2c2_dataset.pdf}
% \vspace{-4mm}
\caption{{MI AUC reported over training time for different entities in the i2b2 dataset.}}
\label{fig:i2b2_mia}
% \vspace{-5mm}
\end{figure}


% \dali{we definitely need a second (or may be even a third use case), whether it is phone numbers, names, Social security numbers, etc... ).} 

% \section{Use Cases}


% \paragraph{Text Classification Models}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Secret Redaction: Known Surrounding Sentences}
\label{subsubsec:i2b2_secret_redaction}
In Section~\ref{subsubsec:secret_types}, we observed that secrets such as passwords can still be inferred even if there are other labels in the private dataset with the example of the GUM corpus. To give more credence to this observation, we augment the i2b2/UTHealth dataset with phrases containing passwords. This mimics the scenario where the updated NER model is also responsible for redacting credentials for controlling access to medical records.
%, we wish to measure the potential for these passwords to be leaked by membership inference. 
%For this we consider a setting whereby a model holder has used a set of data to train a NER model for redaction, following this step, the sensitive information redacted training data is accessible by an attacker, whether as an insider, or a separate entity with data sharing agreements. 
As before, we assume that the attacker is able to use the exact surrounding sentence on what may be a secret (password) to perform membership inference on a dictionary of candidate secrets.

To test this scenario, we sample two sets of 150 passwords to serve as our member and non-member set. We then craft a single phrase ``The secret phrase is ****'' to precede all passwords. The phrases with member passwords are then inserted into the i2b2/UTHealth training data to update the spaCy NER model. With both the member and non-member set, the AUC of MI is computed. This experiment was repeated reducing the passwords within the training set (150 to 100, 50 and 30). All experiments were repeated 10 times for an average result. We also report the testing F1-score to evaluate the performance of the trained model (and note that no overfitting has been observed).

% To test this scenario, we: \ben{Rana, to fill in }
% \begin{enumerate}
%     \item Generated two equal sets of passwords from a public dictionary with 150 passwords each.
%     \item Created phrases including each password, i.e., "The secret phrase is *****".
%     \item Included the phrases from 1 set into the  training data of the i2b2UTHealth challenge dataset, we consider this as a member set.
%     \item Updated the pre-trained spaCy NER model with the update set.
%     \item Using the other set of passwords initially generated, measured the AUC of the MI attack at each training epoch.
%     \item Repeated this process 10 times to get an average result.
%     \item We performed the same experiment by lowering the amount of passwords used during training with 100, 50 and 30 passwords.
% \end{enumerate}



% \begin{figure}[t]
% \includegraphics[width=\linewidth]{plots/AUC_SECRET-30-50-100-150_i2b2_n2c2_dataset.pdf}
% \vspace{-6mm}
% \caption{MI AUC for each training epoch with differing numbers of training secrets inserted into the i2b2 dataset. Potential secrets are queried with the same surrounding sentence used in the training process.}
% \label{fig:same_phrases_main}
% \vspace{-5mm}
% \end{figure}

\descr{Results.} From Figure~\ref{fig:same_phrases_main}, we observe that the MI attacker can successfully infer membership of passwords. Furthermore, the ability to infer passwords increases with smaller number of examples in the training dataset (SECRET-30 vs SECRET-150), which is consistent with the observation around the CONTACT label in Figure~\ref{fig:i2b2_mia}. We also observe that the F1-score for the whole model (on the medical dataset) as well as on the SECRET label is high (close to 1.0). This is in contrast with the GUM corpus (Section~\ref{subsubsec:secret_types}, Figure~\ref{fig:rank_wrt_epoch_gum}) where a high F1-score was illusive. This shows that memorization is occurring even when the model is not overfitted. The individualized MI AUC, NER training loss and individual F1-score with standard deviation bands of the different entities in Figure~\ref{fig:same_phrases_main} are shown in Figure~\ref{fig:full_i2b2_secret_loss} in Appendix~\ref{app:full_docredact_loss}.    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Password Redaction: Unknown Surrounding Sentences}
\label{sub:unknown-surround}
Until now we have assumed that the attacker knows the surrounding sentences of the target secrets. We consider the setting where the attacker does not know the exact surrounding sentences used in the private dataset. Note that this is no longer membership inference, but rather an attribute inference attack. 
%Consider the exceptional circumstance whereby a model holder only releases their model as a service to the public, no redacted documents previously used in the training of this model is to be known. Additionally, newly created documents are forbidden to include these training phrases as to avoid a collision with the training data.
We achieve this by repeating the experiment from Section~\ref{subsubsec:i2b2_secret_redaction}, but instead of a single phrase preceding the secret, we craft four distinct phrases for passwords in the member set: (``My secret is ****'', ``The password to my account is ****'', ``Here is the password: ****'', ``Log in using the password: ****''). Each password in the training dataset is randomly assigned to one of the four phrases. On the other hand, the non-member passwords have a different phrase ``The secret phrase is ****''. We also assume that the attacker uses this phrase as the surrounding sentence.

% To test this scenario, we sample two sets of 150 passwords to serve as our member and non-member set. Next, we craft phrases in which a member set password would follow (``My secret is'', ``The password to my account is'', ``Here is the pass:'', ``Log in using the pass:''). We then use a different phrase ``The secret phrase is ****'' to precede the non-member passwords. The member phrases and passwords are inserted into the i2b2UTHealth training data to update the spaCy NER model. With both the member and non-member set, the AUC of MI is computed. This experiment was repeated with a lower number of passwords within the training set (150 to 100, 50 and 30). All experiments was repeated 10 times to obtain an average results. We also report the training loss and the F1-score on a training dataset to evaluate the performance of the trained model (and note that no overfitting has been observed).

% To test this scenario, we: \ben{Rana, to fill in, also give examples of phrases }

% \begin{enumerate}
%     \item Generated two equal sets of passwords from a public dictionary with 150 passwords each. We consider one to be a memberset used for training and a non-memberset used for testing.
%     \item Created phrases including each password using a set of random phrase, i.e., 'My secret is', 'The password to my account is', 'Here is the pass:', 'Log in using the pass:' whereby each phrase is preceded with a password from the memberset.
%     \item Used a single phrase for the non-memberset depicting an attacker using a common template used when sharing passwords, i.e., 'The secret phrase is ****'.
%     \item Included the phrases created using the memberset into the  training data of the i2b2UTHealth challenge dataset.
%     \item Updated the pre-trained spaCy NER model with the update set.
%     \item Using the phrases from the non-memberset, measured the AUC of the MI attack at each training epoch.
%     \item Repeated this process 10 times to get an average result.
%     \item We performed the same experiment by lowering the amount of passwords used during training with 100, 50 and 30 passwords.
% \end{enumerate}

\begin{figure*}[t]
\centering
\begin{subfigure}{0.49\linewidth}
\centering
\includegraphics[width=0.99\linewidth]{revised_plots/AUC_SECRET-30-50-100-150_i2b2_n2c2_dataset.pdf}
% \vspace{-3mm}
\caption{{Same surrounding sentence as training.}}
\label{fig:same_phrases_main}
% \vspace{-5mm}
\end{subfigure}
%
\begin{subfigure}{0.49\linewidth}
\centering
\includegraphics[width=0.99\linewidth]{revised_plots/AUC_RANDOM_TRAIN_SAME_TEST_SECRET-30-50-100-150_i2b2_n2c2_dataset.pdf}
% \vspace{-3mm}
\caption{
{Different surrounding sentences than training.}}
\label{fig:diff_phrases_main}
% \vspace{-5mm}
\end{subfigure}
\caption{MI AUC for each training epoch with differing numbers of training secrets inserted into the i2b2 dataset. Potential secrets are queried with surrounding sentences. The overall F1 score was computed on testing data. }
% \vspace{-3mm}
\end{figure*}


% \begin{figure}[t]
% \includegraphics[width=\linewidth]{plots/AUC_RANDOM_TRAIN_SAME_TEST_SECRET-30-50-100-150_i2b2_n2c2_dataset.pdf}
% \vspace{-6mm}
% \caption{
% % AUC reported over training epochs for different numbers of training secret entities with inserted into the i2b2 dataset. This experiment queries a secret with a surrounding sentence different from the surrounding sentences used in the training process.
% MI AUC for each training epoch with differing numbers of training secrets inserted into the i2b2 dataset. Potential secrets are queried with a different surrounding sentence than those used in the training process.
% }
% \label{fig:diff_phrases_main}
% \vspace{-5mm}
% \end{figure}

\descr{Results.} From Figure~\ref{fig:diff_phrases_main}, we observe that the performance of MI on unseen surrounding sentences is close to a random guess (0.5 AUC). This observation is not significantly influenced by the number of samples present in training the secret class in contrast to prior results. However, we note that the F1 score of redacting secrets has degraded to 0.65, with the use of different surrounding sentences in the test set to those in the training dataset (c.f. Figure~\ref{fig:same_phrases_main}), irrespective of which secrets were used.

The performance of the NER model is decreased if it has not previously seen a surrounding sentence during training. Thus, the training process should contain sufficiently many representations of expected surrounding sentences for better accuracy. On the contrary, the attack is more successful if the attacker can craft surrounding sentences that are similar to the ones used in the private dataset. For instance, an attacker may employ a strategy to recover a sufficiently similar surrounding sentence (by checking if the redaction accuracy of the updated NER model increases on a generic secret), prior to performing the membership inference attack on the target secret. For instance, for the case of phone numbers, the attacker could craft a phone number distributed similar to the original data (e.g., a US mobile phone number). The attacker can then query multiple manually crafted sentences with this phone number, e.g., ``Please call me on ..., My phone number is ..., ... is where you can reach me.'' With each subsequent query, the surrounding sentence with the highest probability can be further perturbed by replacing words that increase the confidence of the whole sentence. The idea being that the manually crafted surrounding sentence closest to the actual surrounding sentence would give the highest confidence by virtue of being in the training dataset. Figure~\ref{fig:same_phrases_main} shows the plausibility of this approach. 
% we could speculate a secret in the same distribution, but not specifically inthe training data
% 14:57
% e.g. phone numbers
% 14:59
% e.g.
% Please call me on <Phone Number>
% My phone number is <Phone Number>
% <Phone Number> is where you can reach me
% With the highest confidence, more minor alterations could be made
% My phone number is <Phone Number>
% My mobile number is <Phone Number>
% My digits are <Phone Number>
% <Phone Number> is my phone number
% 15:00
% we do have evidence working against this tough, in our defence experiment with replaced secrets, the F1 is much lower for the entitiy, but we have no evidence for the surroudning text
% One potential approach could start with the manual crafting of multiple viable sentences surrounding a sensitive information placeholder. With each subsequent query, the highest probability surrounding sentence is further perturbed by replacing words that increase the confidence of the whole sentence.}
However, we defer detailed investigation of the impact of similar surrounding sentences as future work. 

%\hassan{Example to be provided here: Section 4.3, how an unknown surrounding sentence could be reconstructed exactly?
%We shall provide an extended example in Section 4.3, whereby an attacker could perform a masked word cloze task to generate parts of a surrounding sentence, the intuition that higher confidence words (for the surrounding sentence) are likely to be in the training dataset holds.
%}

%Fortunately, the secret class is able to learn generic password characteristics independent of the phrase, as observed in the increasing secret-F1 score. This is a good outcome for leveraging NER models in secure settings, however, this is in direct competition with the information an attacker is is able to obtain, as we have seen previously an attacker with the phrase preceding the secret can in fact infer membership of a password.

%We additionally observe the F1 score of redacting secrets to have been degraded to 0.65 with the use of different phrases to the those in the training dataset (c.f. Figure~\ref{fig:same_phrases_main}), irrespective of which secrets were used. As a consequence and attacker may employ a strategy to first recover a sufficiently similar surrounding sentence (as indicated by an increase in accuracy of successfully redacting a generic secret), prior to performing the membership inference attack on potential secret.

%In this setting, with the context of the redaction classes, an attacker may guess what the surrounding phrase to a secret could be, getting close to what was used, but not exactly.

%*We do not observe any significant overfitting in the secret class and are unable to comment on the performance of MI on dissimilar phrases in an overfit model


==> MI-text classification - PETS 2023/introduction.tex <==
\section{Introduction}

Language models (LMs) are statistical models that assign probabilities to words to perform different natural language processing tasks~\cite{carlini2020extracting, hoang2019efficient, lample2016neural, bengio2003neural}.
LMs are trained on large datasets, and over the years, their model architecture has become substantial with 350 million~\cite{devlin2018bert} to over 100 billion parameters~\cite{radford2019language, brown2020language}, which increases the model's ability to learn the language and fluently generate text. At the same time, it has been shown that LMs are susceptible to membership inference~\cite{carlini2019secret, carlini2020extracting, zanella2020analyzing, song2019auditing}, whereby it is possible to tell if a given text was used in the, potentially sensitive, training dataset. Membership inference is a general attack on machine learning models and was first introduced by Shokri et al~\cite{shokri2017membership}. 

Membership inference attacks in LMs have predominantly been demonstrated on the task of \emph{text prediction}~\cite{carlini2019secret, carlini2020extracting}, e.g., predicting the most probable word given a sequence of words. 
In this paper, we instead study membership inference attacks on the language problem of \emph{text classification}~\cite{lample2016neural}, where the model classifies tokens in a given text sequence into classes or labels. 
%\dali{Narrowing down the topic or the type of models we are interested in is Fair enough. However, this is kind of not adequately presented in the context of the privacy risks we have just introduced in the previous sentence}
More specifically, we target named entity recognition (NER), which is a task in information retrieval used to identify and label chunks of data appearing in unstructured text into predefined categories or labels~\cite{nadeau2007survey}. Our focus on NER models is motivated by its increasing potential for use in applications involving sensitive data. NER models have been used to categorise medical entities (e.g., drugs) in unstructured medical data~\cite{habibi-med-ner, ge2020fedner}. Similarly, NER models have been proposed to automatically identify sensitive information to prevent data leaks~\cite{gomez2010data}, and in a similar application of automatically redacting sensitive information from documents before sharing~\cite{kanchana2020optical}, which is otherwise a highly manual and laborious task requiring domain expertise~\cite{gordon2013mra}. NER models have also been proposed to automatically de-identify patient notes in electronic health records~\cite{dernoncourt2017identification}. In a contemporary use case, these models have been proposed to de-identify sensitive information from COVID-19 data before sharing and publication for research purposes~\cite{ner-covid}. The underlying data in these uses of NER models is highly sensitive. If this data is used to {(re-)train} an NER model, then one would hope that the model is not susceptible to membership inference. 

%\dali{Until now, many things are still not clear... The most important one being WHAT THe problem we are addressing is?? I think we are missing the WHAT and HOW in the introduction AND even to some extent in the Abstract. I would like that we clarify whether we are addressing the problem of possible MIA in NERs using two techniques or a different high level attack? And then the WHY Would be clearer from the implications of the attacks on NER models.}


More elaborately, our scenario is when a service provider builds on top of an off-the-shelf NER model, pre-trained on a large public corpus, by updating the model using its own, potentially sensitive, private dataset in order to expand the set of named entities (labels) for specialized tasks. This scenario  reflects real-world use of NER models, as often they are pre-trained on a large corpus, and hence both the pre-trained model and the corpus is public information. However, the re-training of the generic model maybe for more specific applications, such as redaction of sensitive information, in which case the private dataset may be sensitive.
%\dali{What is really unclear is WHY we are considering this use case / assumption? The reader would have not clue at this stage.} 
These specific applications may include examples listed above, e.g., identifying medical entities and redaction of sensitive information. The resulting model is then made available as an online service for customers to query in a black-box manner. A query is the customer's document which she would like to process. For example, a document for automatic redaction of sensitive text. The output is the processed document in the form of identified labels for each token and their probability scores.\footnote{See Section~\ref{sec:MIA_memorization} for the precise definition of the input and output.} We investigate the susceptibility of this private dataset to inference attacks.    

We choose spaCy~\cite{spacy} as a representative of NER models, which is an open-source natural language processing library based on neural architecture~\cite{lample2016neural}. Two components of spaCy are common across a wide range of NER models~\cite{yadav2019survey}: a tokenizer, that accesses an internal vocabulary, and the neural network (NN) based NER component, which takes input from the tokenizer and outputs labels. See Figure~\ref{fig:spacy-updated-ner}. When the spaCy NER model is updated with new training data, both the vocabulary and the NN model are updated. The updated vocabulary contains any new words contained in the training data. In this paper, we demonstrate two membership inference attacks on NER models with the spaCy NER model as a use-case. 



The first attack exploits the NN model, and demonstrates that membership of sensitive words, such as passwords and credit card numbers, can be inferred even when they occur in the training model only once~\cite{feldman2020does}.
% \dali{Is it "even when" or "in particular when"/ According to the paper "Does Deep Learning Require Memorization?" (STOC 2020) the memorization is happening because of these single occurences of labels in the training set... Regardless I thin we should cite that paper here as it is a PET Award 2021 and it strengthens the rationale of our attack} \rana{even when because we also have cases where we train the model with more than one password. I'm citing the paper at the end of the last sentence.}. 
This phenomenon is related to unintended memorization in NNs. While unintended memorization has been demonstrated in NNs in general including text prediction models~\cite{carlini2019secret, carlini2020extracting}, our results show that the spaCy NER model is particularly vulnerable to this attack. We first demonstrate membership inference using a password use-case, where the NER model is updated with a single phrase containing a secret word, i.e., password (cf. Section~\ref{sec:MIA_memorization}). We use an existing membership inference algorithm from Salem et al.~\cite{salem2019ml}. The novelty is the first demonstration of this attack on NER models. Our results show that an attacker with a dictionary of passwords, one of which is the target password, can successfully infer the target password even when the phrase is only included once (to update the NER model), clearly demonstrating memorization of the NN model. Within Section~\ref{sec:MIA_memorization}, we also measure how different parameters have a direct impact on the degree of memorization, including the %model architecture, 
strength (entropy) of the memorized password, and number of insertions of the same password into the training data. Additionally, we demonstrate this memorization generalizes beyond passwords to phone numbers, credit cards and IP addresses. We also demonstrate that it is possible to infer words close to the secret words, which helps an attacker find the target password even when it is not in her initial dictionary of possible passwords. This is known as attribute inference in the literature~\cite{yeom2018privacy, zhao2021feasibility}. Next we demonstrate our attack on a practical use-case of document redaction, whereby the NER model is updated on a publicly available medical dataset, which we assume to be a private dataset. We show that an attacker with access to the NER model can successfully infer membership (cf. Section~\ref{sec:doc-redact}).
%Furthermore, compared to the previous version of spaCy, the latest version (version 3.0.3 at the time of this writing), is more prone to unintended memorization .
% \dali{Do we provide explanations later on about WHY it is the case? i.e. what changes happened in the model so that it became more prone to memorization?}. \rana{No concrete facts, however they have a transformer based model requiring GPU but it hasn't been used for the experiments in this paper.} 

The second attack is a \emph{timing-based side-channel attack} which exploits the difference in execution paths when the NER model is queried on a text containing a member word (in the training data) versus a non-member word. This attack exploits the tokenizer, and is specific to NER models which use a vocabulary. This feature differentiates NER models from other machine learning models where, from a black-box point-of-view, there is little difference in execution paths between a member and a non-member sample. 
%Nevertheless, our attack shows that side-channel attacks may have applicability in other instances of machine learning as a service.
%We demonstrate the unintended memorization of training data of NNs in the NER model implemented within the spaCy library.
Finally, by exploiting the difference in execution paths of the NER models when processing member secrets in the training data and non-member text, our timing attack can infer the member secrets used to update the NER model (cf. Section~\ref{sec:MIA_timing}) with an AUC of 0.99.


% \ben{Add a reference that NER is used extensively in medical records: see Draft dent by Dali}~\cite{settles2005abner}

Next, we introduce preliminaries and define our threat model in Section~\ref{sec:background}. 
In Section~\ref{sec:MIA_memorization}, we demonstrate the unintended memorization of the NER model and show our first membership inference attack against the NER models by exploiting its memorization. We then present the experimental results of our membership inference attack on NER models for document redaction use-case in Section~\ref{sec:doc-redact}.
In Section~\ref{sec:MIA_timing}, we present our NER model membership inference attack exploiting a timing side-channel and then discuss its experimental results. We propose potential defences for both attacks in Section~\ref{sec:defences}. We review related work in Section~\ref{sec:related_work}. 
% Finally, Section~\ref{sec:conclusion} concludes the paper. 


% To demonstrate our attacks We experiment with spaCy~\cite{spacy}, a natural language processing library that provides a model based on neural architecture~\cite{lample2016neural} to perform NER task that assigns labels to contiguous token in a given text. The default model is trained to identity common labels including person, organization, location etc., but also giving its user an ability to add more labels and train the model by providing their own examples. 
% Machine learning models however, are also known to leak information~\cite{shokri2017membership,salem2019ml} about training data which could include private information, more specifically the memorization of private information in language models~\cite{carlini2019secret, carlini2020extracting, zanella2020analyzing, song2019auditing} have brought serious privacy concerns in machine learning.
% It all started when Shokri et. al first introduced the {\it membership  inference} attack on machine learning models where an adversary could predict whether a certain data sample was used in the model's training data~\cite{shokri2017membership}.

%In this paper, we specifically target a language problem of text classification~\cite{lample2016neural} where the model is tasked to classify tokens in a given text sequence to classes/labels, where a use case could be used for identify sensitive information in a given text. Over the past few years, a lot of work has been done and patents have been released for the process of identifying valuable information within a text document in an automatic fashion~\cite{pearl2016data}, from simple word search, regular expression matching and huge dictionary search~\cite{googledlp2017} and now with Natural Language Processing that more formally is known as named entity recognition or NER. NER is one of the tasks in information retrieval that is used to identify and label chunks of data the appear in a given text into predefined categories~\cite{nadeau2007survey}. Generally, NER models are trained to identify and assign predefined labels to a given word or multiple words. The ability to train such models to identity sensitive information that could then be used to efficiently redact information from the given text~\cite{kanchana2020optical}. 

%\textbf{Motivation}
%


%NER system has been used to identity sensitive information in various settings~\cite{gomez2010data, ge2020fedner, kanchana2020optical} and hence has pose a risk to the sensitivity of the data used during training. It is because this personalized training of the model requires company data, we show in our initial experiments, that the update set used to train the model would be susceptible to membership inference attacks.

% If the model is updated with a training set whereby the same piece of sensitive information occurs a significant number of times, the model is able to memorize the sensitive information. Consequently, leading to an attacker finding membership information, and even potentially recovering the sensitive information. 
% It is very likely that such sensitive information repeats itself in the training set, for example user emails may be at risk, when redacting emails, with repeated emails, the model is repeatedly exposed to the sender's signature block which is very likely to include personal information of the sender.

% \tham{Problem with neural architecture of the NER model related to memorization and attribute inference attack here}

% \tham{Side channel attack here} 
% Membership information of a given text in the training data can be revealed by exploiting the time the model takes to return prediction on a query text. We observe the fact that a model takes less time to process a query if the text was in the training data. The side channel attack targets the updated NER model to infer the private dataset that was used to update the model.  


% \paragraph{Threat Model}.


%The ability to train such models to identity sensitive information that could then be used to efficiently redact information from the given text~\cite{kanchana2020optical}.




%\hassan{We may skip the following}
% We make the following contributions:
% \begin{itemize}
%     \item We demonstrate that the neural network used in language models unintentionally memorizes the private information which makes it prone to attribute inference attacks where adversary can infer sensitive attribute of the model's input in the inference phase. 
%     \item We then evaluate the proposed attack on document redaction application where the adversary could infer some redacted text was in the training data and propose an algorithm to partially extract/recover the redacted text in the document. 
%     \item We demonstrate side channel attacks on a target NER model to infer the presence of words in the training data. We exploit time difference in the model when making predictions on seen words (during training) compared to unseen words. 
%     \item We propose defense mechanisms for both attacks.
% \end{itemize}

% The organization of the paper is as follows. 

% \hassan{The following text can be condensed and moved elsewhere}
% Previously, the redaction of sensitive information from documents is a highly manual task requiring expertise and many hours to complete~\cite{gordon2013mra}. One of the major problems with redaction is that it can't be always content based, and for redacted information based on context more sophisticated process are required and as more documents are being generated, proposals have been made to automate document redaction to provide cost and time savings for the privacy-conscious document holder using text classification algorithms in natural language processing; However with the use of machine learning techniques for effective text classification, and subsequently text redaction may lead to privacy risks for the data used to train the models. To identify sensitive information, sensitive information would be used to train models, particularly if a model is to be tailored for a specific set of policies, a personalized process for each different company. 

==> MI-text classification - PETS 2023/memorization.tex <==
\section{Membership Inference via Memorization}
\label{sec:MIA_memorization}
% \hassan{We need a threat model here together with a diagram. The initial public NER model is updated with new information using some sensitive information and that is made available either as a public API (black box) or as a product (white box setting). The attacker would like to then infer information about the dataset used in the update.}

% \dali{Don't we need a more generic threat model, i.e. applicable to both Memorization and Side channel attacks. We can refine them when addressing each attack...}


%In this paper, we show that (updated) NER models are susceptible to two membership inference attacks. The 
Our first attack, which is the subject of this section, targets the updated NN model (see Figure~\ref{fig:spacy-updated-ner}). More specifically, we demonstrate that the updated NN model memorizes information from the private dataset which could be inferred by querying the updated NER model. We essentially use the observation from previous membership inference attacks such as~\cite{shokri2017membership, salem2019ml, carlini2019secret} that machine learning models are more confident in predicting inputs used in training versus unseen inputs. Translated to the NER case, this means text used in training (i.e., from the target dataset) is likely to be given higher scores than text never seen by the NER model. In the following, we first demonstrate the feasibility of this attack using simple phrases containing different secrets, e.g., passwords and credit card numbers, within the training dataset to update the NER model. Section~\ref{sec:doc-redact} broadens the attack to cover sensitive information in the more practical scenario of document redaction. We emphasize the exploratory nature of this section as we delve into the extent of, and reasons behind, memorization in NER models; hence the use of simple phrases. Section~\ref{sec:doc-redact} considers more realistic scenarios where the target secret within one of the phrases is interspersed with other phrases in a large private dataset. Thus, the instances of memorization in this section are not just due to the small size of the private dataset. 

%Having introduced the privacy risks involved with text classification models used specifically for documents redaction tasks, we now describe the experimental methods used to evaluate the memorization and exposure of sensitive information which could further lead to uncover the redacted information of texts used for training of the model. We experiment with the pretrained language models provided by spaCy.

%\subsection{Overview}
%\paragraph{Threat model} For the inference of training data we consider a black-box setting, given the adversary access to the NER model, which is an updated version of the original public NER model. The adversary would then try to infer by querying the updated NER model whether a data sample was used in the training set of the updated NER. The adversary would have access to the score assigned by the model to the targeted class label that the word gets assigned to by the model which would be sufficient enough to make an inference.




%\subsection{Inferring Passwords}
\subsection{Methodology}
\label{sub:method}

We first update the NER model with a single phrase containing some secret information, e.g., ``Alice's secret is qwertyui.'' Specifically, with formalization from \cite{carlini2019secret} demonstrating memorization in text generative models, we construct sentences of the form: $s[r] = \text{``Alice's secret is } r\text{''}$. Here $r$ is a variable representing members from the secret space $\mathcal{R}$. For example, $\mathcal{R}$ can be a dictionary of passwords, with an example phrase $s[ \text{``quertyui''}] = \text{``Alice's secret is quertyui''}$. The remaining text in $s[r]$, i.e., minus $r$, is what we term the \emph{surrounding sentence}. 
The updated NER model is then made available as a black-box service to customers to identifying and redacting secrets in their own documents. 
For instance, given an input ``Bob's secret is 123456'' the NER will label ``Bob'' as a \textit{PERSON} and ``123456'' as the \textit{SECRET}. The user can then choose to redact all \textit{SECRET} label words, resulting in the redacted text ``Bob's secret is $\blacksquare$.'' We assume the attacker can query the updated NER model with secret $r$ and phrases $s[r]$ chosen from a secret space $\mathcal{R}$, and any surrounding sentence.
We also permit the surrounding sentence to be empty, whereby the attacker queries directly with $r$. 
We call the secret the attacker attempts to extract from the private dataset used to train the updated NER model, the \emph{target} secret. The security issue here is the attacker is able to associate a (redacted) password to a user, even though the password is already in the attacker's dictionary.  

\subsection{Evaluation Metrics}
\label{sec:eval-metrics}
%\label{evaluation_metrics}
\descr{Rank.} To evaluate the success of the attack, we rank the scores returned by the NER model for each phrase $s[r]$. Note that the surrounding sentence of the phrase remains fixed, and only change $r$. With lower target secret ranks, the attack is more successful. Specifically, let $\Pr(s[r])$ denote the probability score assigned to secret $r \in \mathcal{R}$ by the NER model when queried with text $s[r]$. Then, the (normalized) rank of the secret $r$, is:
\[
\textbf{rank}(r) =  |\{r' \in \mathcal{R} : \Pr(s[r'])\geq \Pr(s[r])\}|/|\mathcal{R}|,
\]
where $r'$ are the other possible secrets in the search space $\mathcal{R}$. The rank lies in the range [0, 1], where $0$ means no other secret in $\mathcal{R}$ has higher (probability) score, and $1$ means the probability score is lowest among all $r \in \mathcal{R}$. 

\descr{Password strength (entropy).} 
In addition, for the specific case when the secret is passwords, we also use the \texttt{zxcvbn} password strength estimator~\cite{wheeler2016zxcvbn}, as a proxy for entropy of passwords to evaluate attack success as a function of password strength. 
\texttt{zxcvbn} estimates password entropy by matching password sub-parts with known patterns, e.g., words, sequences, and dates, scoring the matched patterns and using the entropy to further estimate the number of guesses an attacker would need to crack the password.
\texttt{zxcvbn} defines password strength on a five level scale $[0-4]$ increasing from 0 to 4, to define categories for the number of guesses required to crack the password in orders of magnitude. Specifically, strength scores 0, 1, 2, 3 are assigned to passwords that require less than $10^3$, $10^6$, $10^8$, $10^{10}$ guesses respectively, whereas strength score 4 is assigned to those that require at least $10^{10}$ guesses.
%\dali{Why we did not analyse MIA success as function of the actual entropies? Why do we have to rely on the classes/score this tool provides ? Besides, it feels this would be completely reliable on the way entropy is calculated without knowing what these known patterns are (dictionaries ? how often they are updated, etc... ) } \rana{Instead of directly analysing entropy we use the password strength metric to analyze memorization, this could further be used in the MIA attack we're performing in section~\ref{sec:doc-redact} by maybe adding phrases with controlled strength score and checking for MIA success with equal number of examples for each strength score? 
%\\ We do have to rely on the scores returned by the tool to get the ranks and also perform the MIA, i don't know if this could be done in a different way.}
%\hassan{<-- This is not clear. Level $i$ means that it requires 10 times more guesses than Level $i - 1$? How about Level 0?}

\descr{Levenshtein distance.} When evaluating similar secrets (words) with potentially similar ranks, we use the Levenshtein distance $L$ as a distance metric. We define $L$ for each of the four word features: $L_{\text{prefix}}$, $L_{\text{suffix}}$, $L_{\text{shape}}$ and $L_{\text{norm}}$, and define the feature distance (\textbf{f-distance}), as the sum of the the aforementioned $L$. Thus, the feature distance of two secrets $r, r' \in \mathcal{R}$ is defined as
% We define feature distance as the distance of a secret from the training secret based on the sum of sub-word features including PREFIX, SUFFIX, SHAPE and NORM of a secret. We denote \textbf{f-distance} as the feature distance of two texts. Specifically, for two given texts $r$ and $r'$ the feature distance between them is calculated as the summation the distance between their prefix $L_{prefix}$, suffix $L_{suffix}$, shape $L_{shape}$ and norm $L_{norm}$. 
%\begin{equation*}
\begin{align}
    \textbf{f-distance}(r, r') &= L_{\text{prefix}}(r, r') + L_{\text{suffix}}(r, r') \nonumber\\
    &+ L_{\text{shape}}(r, r') + L_{\text{norm}}(r, r') \label{eq:f-dist}
\end{align}
%\end{equation*}
% \textbf{f\_distance}(r, r') = {L_{prefix}(r, r') + L_{suffix}(r, r') + L_{shape}(r, r') + L_{norm}(r, r')}




%In our experiments, we use spaCy's NER component, which is a trainable component, allowing us to add new classes to the NER system and update the model with user defined examples. The examples that need to be fed to the model before training are required to be annotated by labeling words in the sentence to a corresponding label. 

%We generated random phrases of a specific sequence format $s$ = ``Alice's secret is *****'' where the asterisks are replaced by a secret picked from a randomness space $r$. This method is build upon the existing work in~\cite{carlini2019secret}, by  formally defining the sequence format with a secret information as $s[r]$ which refers that the asterisks are to be replaced from randomness space $r$. That inserted secret $\hat{r}$ is a word or number is randomly picked from the randomness space. For example, a secret could be a random password picked at random from a randomness space as big as a publicly available password dictionary and one such example could $s[\hat{r}]$ = ``Alice's secret is qwertyui''.

% In our experimental methods:

% \begin{enumerate}
%     \item We test out memorization by doing a membership inference attack by first updating the model with a single phrase (e.g., ``Alice's secret is qwertyui'') that contains an out of distribution word (e.g., ``qwertyui'') picked randomly from a set of passwords and then querying the model with the whole set of password to see which password is given the highest probability score.
%     % \item We use the rank metric described in Section~\ref{evaluation_metrics} to rank the passwords based on exposure value, the higher the exposure, the more the model has that word memorized.
%     \item We use the rank metric (Section~\ref{evaluation_metrics}) based on the probability scores assigned to the password in the text to investigate how the memorized word ranks the highest each time.
%     \item To get an average of the rank of the queried password, we run the same experiment on $N$ different passwords (e.g., training the model with 1 password at a time) and to average out for each password we train the model 48 times. The number is picked due to the strictness of resources.
%     \item We tweek the experiments with multiple number of insertions and increasing the number of epochs to see at what point the model completely memorizes the trained sequence. The memorization is shown in figure~\ref{fig:memorization-spacy}.
%     \item We generate passwords to train the model with, using password strength~\cite{wheeler2016zxcvbn} and investigate the level of memorization for different scores of strength.
    
% \end{enumerate}




%\subsection{Evaluation}
%\subsubsection{Evaluation Metrics}
%\label{evaluation_metrics}
%In this section, we will define the metrics used to evaluate the extent of memorization and the privacy risk of sensitive information or an inserted secret in the training data of the model. We adapt the exposure metric from the secret sharer~\cite{carlini2019secret} with slight modifications in context of our setting. Firstly, we define the rank of the inserted secret, this metrics is slight different to the work in~\cite{carlini2019secret} as they used the perplexity scores provided by the model for a given text whereas in our case, we use the probability score assigned to the target class of the secret word/phrase.

%Given a secret phrase i.e. $s[r]$ = ``Alice's secret is qwertyui", including some secret information ${r}$ sampled randomly from a randomness space $\mathcal{R}$. In this example, the secret is a password picked randomly from a list of $\mathcal{R}$ possible passwords from a password dictionary. The rank of the secret is defined as the index in the list of randomly picked $\mathcal{R}$ passwords, ordered by the probability scores assigned to each individual password $s[{r}]$, for a particular known class, in this case ``PASSWORD".
%\\
%\textbf{Metric 1} \textit{The rank of a secret $s$ is then defined as}
%$$ \textbf{rank}(s[r]) = |\{r' \in \mathcal{R} :Pr(s[r']) \leq Pr(s[r])\}| $$
%\\
%Where $Pr(s[r])$ is the probability of the secret $r'$ in the phrase $s$ randomly picked from a randomness space $\mathcal{R}$ where it should be greater than all the other possible secrets $r'$ from the same randomness space.

\subsection{Experimental Results}

To obtain an accurate measure of the rank, we construct $N$ different phrases $s[r]$ each containing a different random target secret $r \in \mathcal{R}$ (but the same surrounding sentence), and update the NER model with only the phrase $s[r]$. The results are averaged over 48 runs for each secret. 
%To allow comparison between target secret spaces of different sizes, we normalize the ranks within the range [0, 1], where $0$ means no other secret in $\mathcal{R}$ has higher (probability) score, and $1$ means the probability score is lowest among all secrets in $\mathcal{R}$.

\subsubsection{Effect of Repeated Insertions}
We use $N = 10$ different target passwords chosen randomly from a space of $|\mathcal{R}| = 2000$ passwords, which in turn are picked randomly from a public password dictionary with one million passwords~\cite{github_passwordlist}.
% \footnote{\url{https://github.com/danielmiessler/SecLists/blob/master/Passwords/Common-Credentials/10-million-password-list-top-1000000.txt}} 
We then measure the rank of each target password averaged over 48 runs. We vary the number of insertions of the phrase $s[r]$ from 1 to 4. The average (normalized) ranks of the target passwords as a function of the number of epochs used to update the NN model are shown in Figure~\ref{fig:memorization-spacy3}. After less than 10 epochs even with a single insertion, the model memorizes the target password (rank of 0). However, we note that there is a minor increase in the memorization when the password is inserted more frequently, but there are diminishing returns. {Additional insertions can be achieved with increased batch size as the likelihood that training samples with a password (sensitive information) is sampled and propagated through the network for training increases, resulting in more memorization.}
%\hassan{Batch Size~Changing batch size is equivalent to altering the number of times a secret is presented to the model during training (Section-3.3.1). We will add this relationship to the text.}

%\hassan{We can remark about the difference in architectures of 2.3 and 3.0?} \rana{Don't have concrete facts to address here so just a general comment}

%Another salient observation is that the ranks of the target secret starts increasing after about 25 epochs, and shows an upward trend as the number of epochs increase further, across all insertions. We speculate that with repeated presentation of the phrase $s[r]$, via increasing number of epochs, spaCy 3 is able to generalize and learn that any token in the same position within the surrounding sentence in $s[r]$ is a secret, thus producing a similar probability score for any secret as the target secret.
%We suspect that given the repeated presentation of the single secret phrase to the model, spaCy 3 is able to generalize and learn that any token in the position following our prefix is automatically a secret, thus producing a similar confidence score for any secret as compared to the confidence of the it's prediction on the original training secret.  \hassan{more commentary? How about spaCy 3 curves showing higher rank later}.

%\tham{Do we also need to show the loss in the graphs in order to say memorization is not due to overtraining?} \rana{TODO-report Loss in Figure 5 and Figure 7}

% \begin{figure}
% \centering
% \begin{tabular}{c}
% %\subfloat[spaCy 2.3.2]{\includegraphics[width=\linewidth]{plots/SpaCy_2.3.2_RANK_PER_EPOCH_AND_INSERTION.png}}\label{fig:spacy2} \\
% %\subfloat[spaCy 3.0.3]{\includegraphics[width=\linewidth]{plots/spaCy3.0.3_RANK_PER_EPOCH_AND_INSERTION.png}} \label{fig:spacy3}
% \subfloat[spaCy 2.3.2\label{fig:memorization-spacy2}]{\includegraphics[width=\linewidth]{plots/RANK_PER_EPOCH_AND_INSERTION_AVERAGED_LINE_PLOT_spacy2.3.2.pdf}}  \\
% \subfloat[spaCy 3.0.3\label{fig:memorization-spacy3}]{\includegraphics[width=\linewidth]{plots/RANK_PER_EPOCH_AND_INSERTION_AVERAGED_LINE_PLOT_spacy3.0.3.pdf}} 
% \end{tabular}
% \caption{The extent of model memorization for out-of-distribution words in two different versions of spaCy. ``Insertions'' refer to the number of times the same phrase is repeated in the training set, ``Epochs'' is the number of training iterations the model undergoes during the update process. ``Ranks'' is calculated using the exposure metric based on the probability score assigned to the label. \hassan{this ficutre should use some subfigure environment -- not tabular}}
% \label{fig:memorization-spacy}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%     \centering
% \includegraphics[width=\linewidth]{plots/SINGLE_RANK_PER_EPOCH_AND_INSERTION_AVERAGED_LINE_PLOT_spacy2.3.2.pdf}
%     \vspace{-2mm}
%      \caption{spaCy 2.3.2}\label{fig:memorization-spacy2}
%     \end{subfigure}
%     %
%     \begin{subfigure}{0.49\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{plots/SINGLE_RANK_PER_EPOCH_AND_INSERTION_AVERAGED_LINE_PLOT_spacy3.0.3_XLIM_10.pdf}
%     \vspace{-2mm}
%     \caption{spaCy 3.0.3}\label{fig:memorization-spacy3}
%     \end{subfigure}
%     \vspace{-3mm}
%     \caption{The extent of model memorization for out-of-distribution words in two different versions of spaCy. ``Insertions'' refer to the number of times the same phrase is repeated in the training set, ``Epochs'' is the number of training iterations the model undergoes during the update process. \ben{To be replotted with smaller width}}
%     \label{fig:memorization-spacy}
%     \vspace{-6mm}
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{plots/SINGLE_RANK_PER_EPOCH_AND_INSERTION_AVERAGED_LINE_PLOT_spacy3.0.3_XLIM_10.pdf}
    % \vspace{-3mm}
    \caption{The extent of model memorization for out-of-distribution words in spaCy (V3.0.3). ``Insertions'' refer to the number of times the same phrase is repeated in the training set, ``Epochs'' is the number of training iterations the model undergoes during the update process.}
    \label{fig:memorization-spacy3}
    % \vspace{-3mm} 
\end{figure}


\subsubsection{Effect of Password Strength}
It is interesting to assess whether memorization is dependent on the strength of the passwords, i.e., high entropy passwords due to being more peculiar than the rest of the words in the corpus might make them more likely to be memorised by the NN model. Indeed, it has previously been shown that words that are \emph{out of distribution} tend to be memorized more than generic words in the case of NN models for text generation~\cite{carlini2019secret}. %Thus, passwords with higher entropy (stronger passwords) could be more prone to memorization. 
To check this, we used the \texttt{zxcvbn} password strength estimator~\cite{wheeler2016zxcvbn} as described in Section~\ref{sec:eval-metrics}. We randomly choose $N = 10$ passwords for each \texttt{zxcvbn} strength level (0 to 4 inclusive), and insert a single phrase $s[r]$ inside the Georgetown University Multilayer (GUM) corpus~\cite{zeldes2017gum} (See Section~\ref{subsubsec:secret_types}) for each of the passwords. These passwords are once again chosen from a list of 2000 randomly chosen passwords $\mathcal{R}$, which itself is a random sample from a public password dictionary with one million passwords. For each \texttt{zxcvbn} strength level, we average the results and investigate the memorization of the model based on the average rank. Based on the results shown in Figure~\ref{fig:zxcvbn_correlation} we observe that complex passwords with a \texttt{zxcvbn} level $4$ take more time to memorize as compared to passwords with lesser \texttt{zxcvbn} level, i.e., $0$ to $3$. There is not much difference, in terms of the rate of memorization, between the first four password strength levels. Moreover, even the strongest passwords (level 4) are eventually ranked 0 by the NN after about 40 epochs. 
%
%shows that the model takes more time to memorize passwords with highest strength \hassan{Not entirely clear: it is showing longer time for strength 4, but strengths 0 to 3 are more or less the same}.
%
%To get an average of the rank of the queried password, we run the same experiment on $N$ different passwords (e.g., training the model with 1 password at a time) and to average out for each password we train the model 48 times. The number is picked due to the strictness of resources.
%
%We experiment the memorization of out of distribution words on two different versions of spaCy. We see that both the versions memorize out of distribution words with high probability, however, the newer release of spaCy shows faster memorization as depicted in Figure~\ref{fig:memorization-spacy}.
{We hypothesize that the passwords contained in strength level 4 are longer, with more internal variation which is not already captured by tokenization. Specifically, the tokenizer may capture general password structures, initially decreasing the rank to ~0.1, but is unable to distinguish between passwords with similar complex structures, thereby requiring additional epochs to memorize the specific digits of the target password.}
%\hassan{I also think that the discussion should be strengthened. For example, fig. 4 shows that passwords with strength 4 have double convergence time when compared to passwords with strengths 0 -- 3. Password with strength 4 needs 10\^10 guess, while passwords with strength 1 and 3 need 10\^3 and 10\^8 guess, respectively. With the bigger gap between strengths 1 and 3, one would expect a bigger gap in convergence time, however, we only see the gap when password with strength 4. Why this behavior arises? 
%
%We believe the set of strength 4 passwords are longer, with more internal variation that is not captured by the tokenization. Specifically, whilst the general structure would capture this internal structure, the exact digits are not, thus requiring more time for memorization (and thus longer convergence)
%
%We will add this hypothesis into the revision.
%}

\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]{plots/RANK_PER_EPOCH_AND_ZXCVBN_AVERAGED_LINE_PLOT_spacy3.0.3.pdf}\label{fig:strength of password}
% \vspace{-3mm}
\caption{It is observed that a higher password strength (as measured by \texttt{zxcvbn}) will take more training epochs before memorization by the NER model as indicated by the near zero normalized rank of candidate passwords.}
\label{fig:zxcvbn_correlation}
% \vspace{-3mm}
\end{figure}


\subsubsection{Effect of Private Dataset Size and Secret Types}
\label{subsubsec:secret_types}
While the above serves as an illustration of the feasibility of the attack, the update process, i.e., using only a single phrase to update the NER model, is arguably not realistic. Furthermore,
we would like to assess the results for secrets other than passwords. To make the training process more realistic, we update the NER model with the Georgetown University Multilayer (GUM) NER corpus which contains around 2,500 annotated documents~\cite{zeldes2017gum}. We include a single secret phrase $s[r]$ into one of these documents. We once again use $N = 10$, and $|\mathcal{R}| = 2000$. We experiment with four different types of secrets: passwords, credit card numbers, phone numbers and IP addresses. 

We generate credit card numbers using Luhn's Mod10 algorithm~\cite{li2011validation} and include a single phrase $s[r]$ in the GUM corpus, which now includes a random credit number as the secret. We calculate the rank the same way as with the passwords by comparing it with 2000 other randomly generated credit card numbers.  
IP addresses are generated by first generating 4 random integers including and between 0 and 255, these numbers are then concatenated together with a ``.'' separating each number (e.g. ``1.10.100.200''). Next, for phone numbers, we randomly generate sequences that follow the following format, ``ddd-ddd-dddd'' whereby each ``d'' is a digit. Special phone numbers as described by the North American Numbering Plan~\cite{nanp} were excluded during the generation process. 

The use of a larger private dataset (GUM corpus), gives us the measure of performance of the NER model, with a training loss, and accuracy via micro-averaged F1 score  (over all ground truth labelled entity word spans and predicted entity spans and entity type labels). The higher the F1-score, the less likely the model is to be overfit to the training dataset. The results in Figure~\ref{fig:rank_wrt_epoch_gum} for all four secret types, show that after a few training epochs, the phrase is memorized regardless of the secret type(in terms of ranks). Comparing Figure~\ref{fig:rank_wrt_epoch_gum} with Figure~\ref{fig:memorization-spacy3} (single password phrase insertion) we see the influence of the larger private dataset, as the speed at which the model generalizes beyond the specific password is delayed due to additional documents for training. This indicates that the model needs to minimize loss on more documents than just the single phrase of Figure~\ref{fig:memorization-spacy3}.
% The use of a larger private dataset (GUM corpus), allows us to measure the performance of the NER model in terms of its training loss, and accuracy via the F1 score (calculated from the precision and recall). The higher the F1-score, the less likely is the model to overfit to the training dataset. The results in terms of the average normalized rank of the target secret is shown in Figure~\ref{fig:rank_wrt_epoch_gum} for the four different types of secrets. The figure clearly shows that after a few training epochs, the phrase gets memorized regardless of the secret. In terms of the effect of the larger private dataset size, comparing Figure~\ref{fig:memorization-spacy3} (single password phrase insertion) with the curve for Passwords in Figure~\ref{fig:rank_wrt_epoch_gum}, we see that the speed at which the model generalizes beyond the specific password is substantially delayed due to the inclusion of additional documents during the training process. This indicates that the model needs to minimize loss on more sentences and documents than the single secret phrase of Figure~\ref{fig:memorization-spacy3}.
Note that the F1 score on GUM test data (Figure~\ref{fig:rank_wrt_epoch_gum}) increases steadily, indicating that the model is not overfitting. The model would typically be trained till a test F1 score around 0.6~\cite{gessler2020amalgum, hou2019few}. 
Note that a random model would have F1 approximately zero as almost all spans would be incorrect. 
% We notice that the F1 score is around 0.5 in Figure ~\ref{fig:rank_wrt_epoch_gum} with a further slow increase on the GUM corpus test set. As the F1 score increases as epochs increase, it indicates that the model is not over-fitting to the training examples and with further training epochs it is expected to reach an F1 score close to 0.6 which is consistent with the F1 score reported in the literature on this dataset~\cite{gessler2020amalgum, hou2019few}.

% \hassan{The following does not explain much. But we need something more here. First, is the curve for passwords between Figures 4 and 5, the same? In which case, adding extra text in the training phase does not do much. If not, what is the difference? Second, why are phone numbers slower to learn? Third, and most importantly, Figure 3(b) shows that the password is learnt after only 10 epochs. Figures 4 and 5 show that the password is learnt after 20 or so epochs. What's the difference?}
% \rana{1. I've mentioned that for the password strength experiment, i also used the GUM corpus, so we see a similar effect. For Figure 3 we didn't use a data set to update the model with. Phone numbers look similar to dates which are part of the training data too, so we have slower memorization because our target phrase containing a phone number is tagged as a secret. It might be tagged as a date of numeric entity before.}
%From this observation, we can infer that the speed at which the model generalizes beyond the specific password to leverage only the prefix is substantially delayed due to the inclusion of additional documents during the training process. The model needs to minimize loss on more sentences and documents than the single secret phrase of Figure~\ref{fig:memorization-spacy3}.


%and figure~\ref{fig:rank_wrt_epoch_gum} quite clearly shows that the phrase with a single credit card number gets memorized and is ranked over other similarly generated numbers.

%\hassan{More discussion here: comparison to Figure 3, why doesn't the curve go up? the difference between different types of secrets}  

%In order to evaluate memorization in a more realistic way, we inserted our target phrase ``The secret phrase is ******* "  that includes our target password in the GUM-Corpus~\cite{zeldes2017gum} by first processing the annotated data into $\leq$ $2500$ data samples and training the pretrained model. We then calculate the rank of our target password by comparing it with a dictionary of 2000 passwords from a public password dictionary. Figure~\ref{fig:rank_wrt_epoch_gum} clearly shows that after a few training epochs, the phrase get memorized.

\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]{revised_plots/RANK_PER_EPOCH_AND_INSERTION_AVERAGED_LINE_PLOT_MULTIPLE_EXPERIMENTS_APPENDIX.pdf}
% \vspace{-3mm}
\caption{With just a single phrase in a training set of 2500 examples, we demonstrate the phrase is still memorized over a short number of training epochs. We see a similar behaviour for different types of secret. Note that the loss line in the graph is overlapping for each of the secret type.}
\label{fig:rank_wrt_epoch_gum}
% \vspace{-5mm}
\end{figure}


\subsubsection{Effect of Similar Secrets}
The analysis in the preceding sections illustrates that if the target secret is within the set of secrets $\mathcal{R}$ available to the attacker, then it is possible to infer the secret via membership inference, i.e., the target secret being of rank 0. In a more realistic scenario, however, the target secret might not be in the set $\mathcal{R}$.
In this case, what does the highest rank secret in $\mathcal{R}$ tell us about the target secret? If the highest rank secret is close to the target secret, then the attacker has at least come close to the target secret. The attacker could then be able to infer the target secret by making small modifications to the candidate with the highest rank in order to ``hill climb'' to the target secret, as we shall see in the next section. 

Taking the password experiment as an example case, we analyzed the model's behaviour for secrets that look similar to the target secret. We first chose $300,000$ initial passwords drawn randomly from the public set of 1M passwords. We then chose $N = 10$ passwords randomly from this initial set. For each of the $N$ passwords, we constructed $70,000$ additional passwords based on three of the four sub-word features (Section~\ref{ner_spacy}) excluding the norm feature (lower case form of the password) as follows: 
%$N = 10$, and $|\mathcal{R}| = 1,000,000$ which includes $S = 700,000$ passwords generated  
%Based on the 3 sub-word features of prefix, suffix and shape, for 1 of the $n$ passwords \hassan{<-- What's $n$ here?}, 
we generate $10,000$ passwords each with (1) the same prefix only, (2) same suffix only, (3) same shape only, (4) same prefix and suffix, (5) same prefix and shape, (6) same suffix and shape, and finally, (7) same prefix, suffix and shape. For (1) (2) and (4) we assume we know the length of the password and add random alphanumeric characters for the rest of the password. For (3) (5) (6) and (7) we use the shape and fill  in missing characters using random alphanumeric characters depending on the characters defined the shape of the target password. These 7 different combinations of sub-word features result in $70,000$ passwords for each of the $N = 10$ passwords, resulting in a total of 700,000 additional passwords. Note that while generating these passwords, we assume that the length of the target password is known. We call these the \emph{feature passwords}, and denote the set by $S$. In total, including the 300,000 initial passwords, we have 1,000,000 passwords in our secret space $\mathcal{R}$. To calculate distance between passwords, we use the \textbf{f-distance} metric as defined in Eq.~\ref{eq:f-dist}. The reason for generating feature passwords is to have more passwords closer to the target password in terms of \textbf{f-distance}. 


We then construct a phrase $s[r]$ for each of the $N$ passwords, update the NER model with this phrase only, and then query the updated NER model with all passwords in $\mathcal{R}$, and record the rank. We update the NER model over 75 epochs, and repeat this procedure 48 times to get an average rank for all passwords. We then normalize the rank between 0 and 1 and sort the results according to the \textbf{f-distance} from the target password. An \textbf{f-distance} of 0 means that it is the target password. As we can see in Figure~\ref{fig:feature_distance_ranks}, the average rank increases as we increase \textbf{f-distance}. This means that secrets (passwords) that are closer to the target secret (password) are ranked highest (closer to 0.0), and secrets further away from the target secret are ranked lower (closer to 1.0).  

%When evaluating against $\mathcal{R}$ passwords, we compute the \textbf{f-distance} for all $\mathcal{R}$ passwords to find passwords that are closer in terms of \textbf{f-distance}. The reason for having the $feature passwords$ is to have more number of passwords that are closer to the target password in terms of $f-distance$. We noticed that these $feature passwords$ rank higher (close to 0) as they're closer to the target password as Figure~\ref{fig:feature_distance_ranks} shows that the further the passwords are, the lower (close to 1) their ranks get.  \hassan{More analysis}


\begin{figure}
\includegraphics[width=\linewidth]{plots/AVG_FEATURE_PASSWORDS_ALL_FEATURE_DISTANCE_RANKS_9_PASSWORD_BOXPLOT.pdf}
% \vspace{-6mm}
\caption{The correlation between the ranks of the words with the \textbf{f-distance} they are away from the target word. }
\label{fig:feature_distance_ranks}
% \vspace{-5mm}
\end{figure}


%To analyze the correlation between the strength or complexity of a word with memorization we experiment with various passwords of different strength. We use \textit{zxcvbn}, a password strength estimator~\cite{wheeler2016zxcvbn} to calculate the strength of a password. Note that \textit{zxcvbn} defines the strength of a password as one of five levels increasing from 0 to 4. 


% \subsubsection{Extracting the Secret}
% \label{sec:extract}

% We now consider the potential of recovering target secrets outside the search space $\mathcal{R}$ of the attacker. Our intuition is simple, secrets ranked higher in $\mathcal{R}$ are likely to be closer to the target secret. From each candidates, the attacker moves closer to the target password by changing a few characters at a time to find higher ranked candidates, iterative moving towards the target password. This is known as an \emph{attribute inference} attack with membership inference attack as a subroutine~\cite{yeom2018privacy, zhao2021feasibility}. 

% This applied to either a Brute-Force (BF) or a hill-climbing approach. With the large character space (lowercase, uppercase, numbers, symbols) BF is prohibitive with more unknown characters, thus the HC approach. Figure~\ref{fig:feature_distance_ranks} demonstrates a clear trend of lower ranks with secret-like passwords, but the curve does not monotonically decrease as a function of \textbf{f-distance}. Fortunately, noisy functions can leverage hill-climbing methods like Simulated Annealing (SA)~\cite{van1987simulated} to approach the target password. SA should reduce the number of queries in contrast to a BF attack. 

% We evaluate both approaches in the scenario where the adversary has knowledge of the last 3 (suffix) and the $1^{\text{st}}$ character (prefix) of the target password. It is assumed that the length of the password is known to the adversary, we only consider character substitutions. SA takes as input, phrase $s[r]$ and outputs the probability score for $r$ by querying the model, it maximizes this score with substitutions to reach the global maxima (the likely target secret). We consider 1-4 missing characters, with 62 (26 lowercase, 26 uppercase, and 10 numbers) candidate characters, it would yield 62, 3844, 238K and 14.7M possible combinations respectively.

% We constrain the number of iterations allowed by the simulated annealing algorithm at 100, with subsequent experiments doubling up to 6400 iterations, a far cry from the 238K combinations of 3 missing characters. 
% We repeat this experiment with 40 different target secrets for each missing character summing up to 160 different passwords, training the model with one secret at once and then running the simulated annealing algorithm for number of iterations specified above. We produce 40 experimental runs for every 1, 2, 3, 4 missing characters respectively.

% The last row of Table~\ref{tab:vary_annealing} shows the performance of the brute force algorithm in finding the missing characters. Noticeably, the algorithm performs best when there are less missing characters (1 or 2), and worse when we have 4 missing characters (only finding the missing characters 5\% of the time). However, among the cases where the algorithm did not find the target password, the exercise was not entirely futile. We notice that when the algorithm found the wrong password, more than 27.5\% of the times for 4 missing characters, the extracted password matched the shape of the target password. Note that the shape tells us whether the missing character is upper case letter, a lower case letter or a digit. Thus, these results show that the adversary can still extract the target password, or at least infer something useful about the target password (e.g., its shape), even when it is not part of the attacker's initial dictionary of possible passwords.

% On the other hand, we note that simulated annealing also performs well for 1 or 2 missing characters, even with a constrained number of iterations. For instance, for 2 missing characters the algorithm is able to find the target password at 33.3\% of the times with only 1600 iterations as compared to the brute force attack which has the success rate of 38.4\% but with 3844 iterations. However, the exact match accuracy of the algorithms is next to 0 for 3 and 4 missing characters. However, this is compensated by recovering the exact shape of the password comparable to the success rate of brute force attack but with a significantly low iterations. For instance, a success rate of 40\% for 3 missing characters with only 3200 iterations (API calls), versus 238,000 iterations in the brute force attack for the same success rate.

% As far as why the two algorithms fare better with lesser number of characters is concerned, we speculate that taking one single character step is still likely producing extremely large changes in the probability score, as seen in Figure~\ref{fig:feature_distance_ranks}, between 2 and 6 distance, the median rank sits at 0.1 relative to the candidate set. When we expand this candidate set to encompass the entire space of combinations of characters, the likelihood we replace a character with one that has a higher probability than the current is even less. The deteriorating results are consistent with the efficacy of attribute inference attacks reported in literature~\cite{zhao2021feasibility}, where it is shown that exact attribute inference is hard as it requires the underlying membership inference attack to be able to distinguish between members and nearby non-members. 


% \begin{table}[t]
% \caption{The Exact and Shape Match Accuracy after performing simulated annealing up to a 6400 iterations and an exhaustive brute force search with passwords that contain 1, 2, 3, or 4 characters missing at random.}
% \label{tab:vary_annealing}
% \centering
% \resizebox{0.95\linewidth}{!}{%
% \begin{tabular}{r|cccc||cccc}
%           & \multicolumn{4}{c||}{Exact Match} & \multicolumn{4}{c}{Shape Match} \\ \hline
% Iterations  & 1         & 2     & 3     & 4     & 1     & 2     & 3     & 4     \\ \cline{2-9}
% 100         & 0.781   & 0.025   & 0     & 0     & 0.937 & 0.615 & 0.15  & 0.05 \\
% 200         & 0.781   & 0.128   & 0.025 & 0     & 0.937 & 0.666 & 0.275 & 0.05\\
% 400         & 0.781   & 0.076   & 0     & 0     & 0.937 & 0.589 & 0.2   & 0.125\\
% 800         & 0.781   & 0.179   & 0     & 0     & 0.937 & 0.769 & 0.25  & 0.1\\
% 1600        & 0.781   & 0.333   & 0.025 & 0     & 0.937 & 0.794 & 0.325 & 0.15\\
% 3200        & 0.781   & 0.358   & 0     & 0     & 0.937 & 0.743 & 0.4   & 0.2\\
% 6400        & 0.781   & 0.333   & 0     & 0     & 0.937 & 0.717 & 0.325 & 0.15\\ \hline \hline

% Brute Force & 0.937   & 0.384   & 0.125 & 0.05  & 0.968 & 0.692 & 0.4   & 0.275  \\ \hline
% \end{tabular}%
% }
% \vspace{-3mm}
% \end{table}


==> MI-text classification - PETS 2023/memorization_based_attack.tex <==
\section{Memorization}
Having introduced the privacy risks involved with text classification models used specifically for documents redaction tasks, we now describe the experimental methods used to evaluate the memorization and exposure of sensitive information which could further lead to uncover the redacted information of texts used for training of the model. We experiment with the pretrained language models provided by spaCy.

\subsection{Overview}

\subsection{Methodology}
\subsubsection{Memorization}
In our experiments, we use spaCy's NER component, which is a trainable component, so we are able to add new classes to the NER system and update the model with user defined examples. The examples that need to be fed to the model before training are required to be annotated by labeling words in the sentence to a corresponding label. 

We generated random phrases of a specific sequence format $s$ = ``Alice's secret is *****'' where the asterisks are replaced by a secret picked from a randomness space $r$. This method is build upon the existing work in \cite{carlini2019secret}, by  formally defining the sequence format with a secret information as $s[r]$ which refers that the asterisks are to be replaced from randomness space $r$. That inserted secret $\hat{r}$ is a word or number is randomly picked from the randomness space. For example, a secret could be a random password picked at random from a randomness space as big as a publicly available password dictionary and one such example could $s[\hat{r}]$ = ``Alice's secret is qwertyui''.

In our experimental methods:

\begin{enumerate}
    \item We test out memorization by doing a membership inference attack by first updating the model with a single phrase (e.g., ``Alice's secret is qwertyui'') that contains an out of distribution word (e.g., ``qwertyui'') picked randomly from a set of passwords and then querying the model with the whole set of password to see which password is given the highest probability score.
    % \item We use the rank metric described in Section \ref{evaluation_metrics} to rank the passwords based on exposure value, the higher the exposure, the more the model has that word memorized.
    \item We use the rank metric (Section \ref{evaluation_metrics}) based on the probability scores assigned to the password in the text to investigate how the memorized word ranks the highest each time.
    \item To get an average of the rank of the queried password, we run the same experiment on $N$ different passwords (e.g., training the model with 1 password at a time) and to average out for each password we train the model 48 times. The number is picked due to the strictness of resources.
    \item We tweek the experiments with multiple number of insertions and increasing the number of epochs to see at what point the model completely memorizes the trained sequence. The memorization is shown in figure \ref{fig:memorization-spacy}.
    \item We generate passwords to train the model with, using password strength \cite{wheeler2016zxcvbn} and investigate the level of memorization for different scores of strength.
    
\end{enumerate}

\subsubsection{Extraction}
To extract the password memorized by the model we propose to target the model's feature extraction layer where the model uses sub-word feature for each word queried to the model. For the extraction of the learned password:
\begin{enumerate}
    \item We analyze the effect of sub-word feature vectors that we have discussed in Section \ref{ner_spacy}. SpaCy uses multiple sub-word features while embedding the words into a context independent vector representation. 
    \item We use a \textit{feature distance metric} to see how passwords, who are close to the trained password rank higher than the password as they move away with respect to those features..
    \item Based on the features of the trained passwords, we generate similar passwords to analyze the impact of features with respect to the distance metrics and the rank.
    \item We formulate an algorithm to extract a password unknown to the adversary by querying the model taking into consideration one feature at a time and getting closer to the target password by finding the passwords with similar features.
    
\end{enumerate}
With the extraction strategy, even if the exact password is not recovered, some features of the password are extracted that reduces the search space of a brute force algorithms by a significant degree.


\subsection{Evaluation}
\subsubsection{Evaluation Metrics}
\label{evaluation_metrics}
In this section, we will define the metrics used to evaluate the extent of memorization and the privacy risk of sensitive information or an inserted secret in the training data of the model. We adapt the exposure metric from the secret sharer \cite{carlini2019secret} with slight modifications in context of our setting. Firstly, we define the rank of the inserted secret, this metrics is slight different to the work in \cite{carlini2019secret} as they used the perplexity scores provided by the model for a given text whereas in our case, we use the probability score assigned to the target class of the secret word/phrase.

Given a secret phrase i.e. $s[r]$ = ``Alice's secret is qwertyui", including some secret information ${r}$ sampled randomly from a randomness space $\mathcal{R}$. In this example, the secret is a password picked randomly from a list of $\mathcal{R}$ possible passwords from a password dictionary. The rank of the secret is defined as the index in the list of randomly picked $\mathcal{R}$ passwords, ordered by the probability scores assigned to each individual password $s[{r}]$, for a particular known class, in this case ``PASSWORD".
\\
\textbf{Metric 1} \textit{The rank of a secret $s$ is then defined as}
$$ \textbf{rank}(s[r]) = |\{r' \in \mathcal{R} :Pr(s[r']) \leq Pr(s[r])\}| $$
\\
Where $Pr(s[r])$ is the probability of the secret $r'$ in the phrase $s$ randomly picked from a randomness space $\mathcal{R}$ where it should be greater than all the other possible secrets $r'$ from the same randomness space.

\subsection{Experimental Results}
We experiment the memorization of out of distribution words on two different versions of spaCy. We see that both the versions memorize out of distribution words with high probability, however, the newer release of spaCy shows faster memorization as depicted in Figure \ref{fig:memorization-spacy}.

\begin{figure}
\centering
\begin{tabular}{c}
\subfloat[spaCy 2.3.2]{\includegraphics[width=\linewidth]{plots/SpaCy_2.3.2_RANK_PER_EPOCH_AND_INSERTION.png}}\label{fig:spacy2} \\
\subfloat[spaCy 3.0.3]{\includegraphics[width=\linewidth]{plots/spaCy3.0.3_RANK_PER_EPOCH_AND_INSERTION.png}} \label{fig:spacy3}
\end{tabular}
\caption{The extent of model memorization for out-of-distribution words in two different versions of spaCy. ``Insertions'' refer to the number of times the same phrase is repeated in the training set, ``Epochs'' is the number of training iterations the model undergoes during the update process. ``Ranks'' is calculated using the exposure metric based on the probability score assigned to the label.}
\label{fig:memorization-spacy}
\end{figure}



==> MI-text classification - PETS 2023/motivation.tex <==
\section{Motivation}
Previously, the redaction of sensitive information from documents is a highly manual task requiring expertise and many hours to complete~\cite{gordon2013mra}. One of the major problems with redaction is that it can't be always content based, and for redacted information based on context more sophisticated process are required and as more documents are being generated, proposals have been made to Automate document redaction to provide cost and time savings for the privacy-conscious document holder using text classification algorithms in natural language processing; However with the use of machine learning techniques for effective text classification, and subsequently text redaction may lead to privacy risks for the data used to train the models. To identify sensitive information, sensitive information would be used to train models, particularly if a model is to be tailored for a specific set of policies, a personalized process for each different company. NER system has been used to identity sensitive information in various settings~\cite{gomez2010data, ge2020fedner, kanchana2020optical} and hence has pose a risk to the sensitivity of the data used during training.

It is because this personalized training of the model requires company data, we show in our initial experiments, that the update set used to train the model would be susceptible to membership inference attacks.

If the model is updated with a training set whereby the same piece of sensitive information occurs a significant number of times, the model is able to memorize the sensitive information. Consequently, leading to an attacker finding membership information, and even potentially recovering the sensitive information. 
It is very likely that such sensitive information repeats itself in the training set, for example user emails may be at risk, when redacting emails, with repeated emails, the model is repeatedly exposed to the sender's signature block which is very likely to include personal information of the sender.



==> MI-text classification - PETS 2023/old_abstract.tex <==
\begin{abstract}

Named entity recognition models (NER), also known as entity identification or entity extraction systems, are widely used for the tasks of identifying named entities (e.g. individuals, locations, drugs, clinical procedures, etc.) in text documents. Machine learning based NERs are often applied to privacy-sensitive applications that need automatic and scalable identification of sensitive information to de-identify personal information and to redact text for data sharing. \dali{add a note on how the training of these models is done? May be an example from the health/medical sector}\rana{We do talk about how the pretrained spacy model is updated with a collection of documents with new entities/labels.}



%\textbf{todo \dali{introduce NER and Machine learning based NERs. Then introduce applications of NER and the privacy perspective}}

%show great promise in many privacy-sensitive applications where they can automatically identify sensitive information in documents to protect against data breaches, to de-identify personal information, and to redact text for data sharing. These applications are inherently trained on sensitive datasets. 

In this paper, we study the case when an NER model is made available to end users as a black-box service identifying sensitive information in their documents and show that these models are vulnerable to attacks inferring information about their training datasets. 


Using the NER model from spaCy~\cite{spacy} \dali{did we use only one model from SpaCy?}\ben{Two versions of Spacy, same provider, slightly different architectures} as a representative implementation, a widely-used open-source natural language processing library, we demonstrate two attacks on these models. 

Our first attack is linked to the underlying neural network (NN) used in the NER model. It demonstrates how to exploit unintended memorization of NNs, a phenomenon NNs are known to be vulnerable to, in the context of NER to \dali{What's the attack objective? What did we demonstrate when exploiting the memorization? in a general sense, not findings specific.}\rana{memorization is exploited for text redaction applications and the ability to retrieve training data information having access to a redacted document used during training}.


Our second attack targets NER models that maintain vocabularies constructed from the training data 
\dali{Speedups of what?} \dali{Can we name these models? i.e. refer to them according to some widely used/accepted terminology...}. \ben{resolved, speedup removed, volcabulary is acccepted terminology}
We show that these models are vulnerable to timing attacks, exploiting the different execution paths taken by words in the training dataset in comparison to words that were never seen by the model. \dali{Same than attack 1. Can we say in a general sense what the attack aims to do. inferring membership in training sets, or some leakage from the training set?? } \ben{Both attacks seek to leak membership information about the training dataset, which in the context of passwords is a security risk, and in the health dataset, a privacy/regulation problem}

We experimentally demonstrate our attacks by updating the public spaCy NER model with phrases containing sensitive information. 

Our results show that the model memorises even when the update contains a single phrase. 

We also demonstrate a membership inference attack \dali{the wording membership inference attack is coming out of the blue here!} \ben{perhaps: We also demonstrate an inference attack to determine the membership of sensitive information contained within the training dataset.} on a document redaction use-case, resulting in more than 70\% AUC. We show that the timing attack is overwhelmingly successful with an AUC of 98.84\%. Finally we discuss some mitigation techniques which can be adopted to make NER models resilient against inference attacks \dali{"some" mitigation techniques is way too vague. I suggest you provide reasonable information about how to mitigate the attacks. If we didn't provide any experimental analysis of the defense techniques, best is to remove this last note}.\ben{we only speculate about defence mechanisms} \ben{perhaps: Finally we discuss potential mitigation approaches to realize the safe use of NER models in light of the presented privacy and security implications of membership inference attacks.}
\end{abstract}

==> MI-text classification - PETS 2023/related_work.tex <==
\section{Related Work}\label{sec:related_work}

% \dali{I think this section needs to be structured as first discussing Attacks against Text Classification models in general, briefly, and then MIA, memorization and side-channel attacks on ML models. This section Should perhaps be moved to the end of the paper and In the Intro, we make our case that this is the first time MIA is demonstrated against Text classification models. }

% Over the past few years, there has been a significant amount of work done in relations to machine learning and privacy.

\textit{Attacks against Text Classification Models.} Recent works have demonstrated a vulnerability of text classification models to adversarial sample attacks, reducing model accuracy or forcing the output of a target label~\cite{liang2017deep, jin2020bert, garg-ramakrishnan-2020-bae}. Garg et al.~\cite{garg-ramakrishnan-2020-bae} propose BERT-based adversarial examples with contextual perturbations from the BERT masked language model, to reduce classifier accuracy by more than 80\%. In contrast, we focus on analyzing the vulnerability of text classification models to membership inference and timing side-channel attacks.

\textit{Membership Inference (MI) Attacks.} With access to a ML model an attacker can determine if a data sample was in the training dataset, or infer its membership, Shokri et al.~\cite{shokri2017membership} first achieved this by training shadow models to mimic the behavior of the target model. Salem et al.~\cite{salem2019ml} proposed a low cost attack on ML models without the need of shadow models, in addition to a relaxed attack that sets a threshold for prediction confidence to identify membership. 
% Following up these initial studies, extensive work on membership inference attacks have been performed under various settings and different ML models. 
On text generation models, Song et al.~\cite{song2019auditing} present a user-level MI attack by training an auditing model that checks the membership of any user sample even if not explicitly used in training the model.
% \rana{Salem et al.~\cite{salem2020updates} infer the information and reconstruct the updated data used for training the model, however this work did not consider language modeling tasks.} 
Salem et al.~\cite{salem2020updates} infers labels of updating data samples and reconstructs the updating data based on output differences between two versions of models. Moreover, this work targets image classification where as our focus is text classification.

\textit{MI Attacks against NER.}
To the best of our knowledge the only work analyzing MI attacks on Named Entity Recognition is~\cite{seyedi2021analysis}. Specifically, Seyedi et al. perform \cite{shokri2017membership}'s Shadow MI attack on a NER model (NeuroNER~\cite{NeuroNER}) used to de-identify medical records. However, Seyedi et al. concludes an inability to distinguish between members and non-members of the medical training data.  
% We remark that NeuroNER~\cite{NeuroNER} has not been updated since 2019.
However, as previously seen in Section~\ref{subsec:MIA_medical_dataset}, contrary to Seyedi et al.'s conclusion, we find there exists a realistic MI threat against the i2b2 medical dataset~\cite{stubbs2015annotating} and when applying MI on sensitive information like passwords.
Furthermore, the NeuroNER model contains a tokenizer, opening potential vulnerabilities to our timing side-channel attack. 
%\tham{todo: add a discussion about the results of our MI attack on the (same) medical dataset with~\cite{seyedi2021analysis}}
% \ben{added}
% \ben{We remark that NeuroNER~\cite{NeuroNER} has not been updated since 2019, and appears to be abandoned.}



\textit{Memorization in Language Models.} Carlini et al.~\cite{carlini2019secret} demonstrate generative text models memorize out-of-distribution secret phrases in the training data and present methods to extract these secrets.
\cite{carlini2020extracting} has recently shown that large language models like GPT-2, trained on text from the internet including sensitive information from billions of users can be attacked to extract personally identifiable information (PII), in extremely large parameter models. Despite these large models demonstrating no memorization through generality tests, they still are capable of leaking information.  
Helali et al.~\cite{helali2020assessing} demonstrates the unintended memorization of NER models specific to labels that share linguistic materials with at least one other label. In this work, we demonstrate that text classification models, specifically Named Entity Recognition models also unintentionally memorize their training data with proposed attacks that exploit said memorization to infer the membership of sensitive information.
Zanella et al.~\cite{zanella2020analyzing} uses differential scores and ranks from two model versions to analyze information leakage of an update set for text prediction tasks.

\textit{Timing side-channel Attacks.}
A timing side-channel is defined as a side-channel that leaks information due to faulty or vulnerable operations of a system~\cite{biswas2017survey}. In literature, numerous timing side-channel attacks have been proposed to attack cryptographic systems. 
% For instance, Onur et al.~\cite{aciiccmez2007cache} proposed a cache-based timing attack on AES software implementation which can obtain the secret keys of remote cryptosystems given that they run on a server with multitasking system and large wordload.
For instance, attacks may exploit delays in memory access of a program due to other programs accessing the same shared memory. Wang et al.~\cite{wang2014timing} proposed an attack to compromise the private key of RSA decryption by monitoring memory accesses. Wang et al.'s attacker continuously issues memory requests to memory shared by the RSA decryption program, measuring the end-to-end delay for request completion. With the delay, the attacker can estimate the number of `1' bits in the RSA's private key. Timing side-channel may also be based on execution time. Chen et al.~\cite{chen2013improving} proposed a timing side-channel attack against the RSA-CRT algorithm that executes a chosen ciphertext attack to collect time measurements on the overall decryption process.  
In neural networks, few works consider the timing side-channel. For instance, Duddu et al.\cite{duddu2018stealing} proposed a timing side-channel attack to reverse the neural network architecture. Specifically, the attacker queries the target model and measures the execution time which is then used to infer the model's depth. 
To the best of our knowledge, our work is the first that exploits the vulnerability of NER models to a timing side-channel for MI attacks.

{
\textit{Contextualizing Differences from Previous Work.} In this work we have shown that NER models are susceptible to membership and attribute inference attacks by exploiting neural memorization and timing side channels. As indicated above, neural memorization has already been demonstrated in the literature~\cite{carlini2019secret, carlini2020extracting}, however their setting is text generation instead of text classification. In the text generation setting, the model returns a ranking of possible word tokens given a sequence of words, which it has learned through its training. Thus, given a sequence such as ``The secret phrase is ...,'' the model returns possible tokens that would complete the sentence. If the model is susceptible to neural memorization, the sensitive word (password in this case) would be higher ranked in the output. From this, a membership inference attack can be launched in a straightforward way. Our text classification setting is different, as the model never suggests tokens, and we need to modify the attack to try different possibilities (e.g., password dictionaries) to guess the missing word (e.g., password).  

We also remark that membership and attribute inference attacks in general need not be related to neural memorization. For instance, membership inference attacks have been demonstrated on machine learning models other than neural networks~\cite{shokri2017membership}. Furthermore, membership inference attacks may use a different exploit other than neural memorization. One such example is overfitting due to over training which is different from neural memorization~\cite{carlini2019secret}. In this paper we have also shown how membership inference attacks can be launched via exploiting side channels, specifically, timing side channels. Note that timing side channels have previously only been demonstrated on stealing machine learning models (model parameters), and not on membership inference on natural language processing models~\cite{duddu2018stealing}. We have shown how this can be done by exploiting the built-in dictionary of member words in NER systems.
}


==> MI-text classification - PETS 2023/threat_model.tex <==
\subsection{Threat Model}
\label{threat_model}
%Language models require regular updates with new data samples to increase the performance of the models. In the case of a Named Entity Recognition system, the 
An NER model can be updated with new samples to identify new named entities (labels). For example, one can update the NER model to enable it to recognise a new named entity `SECRET' by training the model with a private dataset which includes sensitive information such as passwords, emails, phone numbers, and social security numbers. The updating process adds new labels to the initial NER model. We call this the \textit{updated NER} model in the rest of the paper, and the dataset used to obtain the updated NER model as the \emph{private dataset}. The adversary aims to infer information about this private dataset.  

Following the real-world use of NLP models, which often come pre-trained on a large but public corpus, we assume that the pre-trained NER model and its underlying training dataset is public. This also naturally fits our spaCy use case since it is available for download as a pre-trained NER model, which can then be further updated for other applications such as labeling sensitive information. We remark that this assumption is simply to make our setting more natural, as our attacks do not rely on the adversary knowing the public training dataset, and could be applied even if the model was trained from scratch.

We consider an adversary with the following capabilities and knowledge: 

\begin{enumerate}

    \item[A1:] The adversary has black-box access to the updated NER model. 
    \item[A2:] Samples of the (annotated) sensitive information are only introduced in the private dataset (model update).
    \item[A3:] The adversary knows the sentences surrounding sensitive words in the private dataset (However, see explanation below). 
\end{enumerate}

\descr{Justification of Assumptions.} Assumption A1 is the usual black-box setting for membership inference attacks. The adversary can send queries and obtains output from the updated NER model. A query is simply some text to be labelled, and the output is a probability score for each named entity in the input text.

Under Assumption A2, we assume that the private dataset used in the updated NER model contains at least one example of the new sensitive named entity. This example consists of the sensitive information together with the \emph{surrounding sentence}. For instance, the private dataset could be the solitary phrase: ``Alice’s secret is quertyui.'' Here the password ``quertyui'' is an example of the new named entity SECRET. The rest of the phrase constitutes the surrounding sentence. See Section~\ref{sub:method} for further details. We further assume that such examples do not exist in the public training dataset. Indeed, the service provider's goal is to update the NER model for new exclusive services. 

%We consider an adversary with a \emph{black-box} access to the updated NER model (e.g. as a public API query based access). The adversary can send queries and obtains output from the updated NER model. A query is simply some text to be labelled, and the output is a probability score for each named entity in the input text. The adversary aims to infer information about the private dataset. 
%Since the public NER model is available to everyone, we assume the adversary also has access to the public NER model and its underlying public training dataset. \dali{This is the controversial assumption Right? ACTUALLY, it comes out of the blue and we don't necessarily understand why we 're making such a statement and such an assumption. In addition, the assumption that because it is public NER model, that means anyone can have access to the underlying training set doesn't make too much sense to me...  
%Also, where did we say it is a public NER model. We said it's accessible to the public for querying... }

%However, we remark that our attacks do not rely on the adversary knowing this public training dataset. This threat model naturally fits our spaCy use-case as it is available for download as a pre-trained NER model, which can then be further updated for other applications such as labeling sensitive information. 

Assumption A3 states that the attacker additionally knows the surrounding sentence, but not the actual secret, which the attacker would like to infer. This assumption is needed for membership inference. For our main use case of redacting information, the surrounding sentence is not considered sensitive, and thus it can be safely assumed that the attacker would know such text through previously released documents of similar nature. Furthermore, in the same use case, often the surrounding sentence is in a standard format which is easily guessable. For instance, automatic emails with password resets would include some standard text such as ``Your new password is $\ldots$.'' We remark that this assumption is used for the membership inference attack on the NN model, and not the timing-based attack. Nevertheless, we also specifically examine the impact of updating the NER model with different phrases (variants of the surrounding sentence) containing the new named entity in Section~\ref{sub:unknown-surround}. Note that unknown surrounding sentence variant of the attack makes it more of an attribute inference attack~\cite{yeom2018privacy, zhao2021feasibility} rather than a membership inference attack.


%\begin{itemize}
%    \item T2: Black-box query access to the NER model (e.g. API queries)
%    \item T2: Access to the surrounding sentence, but not the actual secret (e.g. access to the redacted documents) \hassan{add that access to surrounding sentence is not required by the timing attack}
%    \item T3: The sensitive class of secrets is introduced in during the model update. \ben{cut this if comment below applies}
%\end{itemize}

%\hassan{Maybe we can label threat model assumptions (T1, T2, etc), and follow each with ``justification''}
%\ben{Is it absolutely necessary to distinguish between pretrained+update, and from scratch models in the threat model? It's a good motivating example for real-world applicability, but in theory there should be only minor differences between them.}

%\rana{We further assume that the adversary has knowledge of the surrounding text of the redacted token. This assumptions holds true for the case when the attacker has access to the redacted documents and tries to infer the redacted tokens using the surrounding non-redacted text.}

%\hassan{Why is this assumption justified? Consider the case of emails where a user's password is reset. In most cases these emails are in standardised format. Thus, we can assume that the attacker knows these phrases.}

%\hassan{The above is to address this comment from reviewer (call it R1): The assumption is that the adversary is supposed to the know rest part of a sentence except the sensitive information it carries. Specifically, the authors assume that the form of a secret carrying sentence is certain and can be represented as s[r]. For instance, s[r]=``Alice's secret is r'', where r is the secret. But the number of different forms is small and those forms are known to the adversary. These small number of s[r] are used to update the public NER models by the victims with their own secrets. Under this assumption, authors demonstrate their success in membership inference of victim's secret.}
% \dali{Not sure what's the intention of having this. Sounds like this should be in the Threat Model section.}

\begin{figure}
\includegraphics[width=\linewidth]{plots/Spacy-ner-Model-Page-3.pdf} \caption{The end to end pipeline of an updated NER model in spaCy. Under a black-box setting, the attacker can query the model by passing text to the \textit{nlp} object, getting labels with their confidence scores.}
% calling \textit{nlp(Text)}}
\label{fig:spacy-updated-ner}
% \vspace{-6mm}
\end{figure}

Figure~\ref{fig:spacy-updated-ner} shows the end to end pipeline for querying the updated NER model with a given text in spaCy. The text is first segmented into tokens by a \textit{Tokenizer} which applies rules specific to each language. %Specifically, unicode text is given to the \textit{Tokenizer}. 
When processing a token, the \textit{Tokenizer} accesses the \textit{Strings} table in the vocabulary (\textit{Vocab}) and checks whether four features of the token including prefix, suffix, shape and norm (lower form) are in the \textit{Strings}. If any feature is not $in$, it is added to the \textit{Strings}. The output of the \textit{Tokenizer} is a \textit{Doc} object which is a sequence of tokens. The updated NER model then processes the \textit{Doc} object and returns the named entities in the input text with probability scores. Note that the updated NER model will take into account the pre-trained word embeddings in the \textit{Pre-trained Vectors} when processing the \textit{Doc} if it is available in the \textit{Vocab}. %For example, given the text ``Alice's secret is qwertyui'', the output of the model will be ``Alice [PERSON, 'score'] 's [O, 'score'] secret [O, 'score'] is [O, 'score'] qwertyui [SECRET, 'score']'', where PERSON, SECRET are predefined named entities, O is assigned for words that are not recognised as any of the predefined named entities of the updated NER model. \tham{repeating the earlier section}

%\paragraph{Black-box setting.} In our threat model, we consider the black-box setting where the updated NER model (i.e. the public NER model is updated with sensitive information) is made available as a public API. The adversary can access to the input and output of the updated NER model only. For a query with a given input \textit{Text}, the adversary can query the updated NER model by passing the input to the \textit{nlp} pipeline. The adversary then has access to the output of the model in the form of a probability score for each named entity in the input \textit{Text}. The adversary aims to infer information about the private dataset used to update the public NER model.

\subsection{Motivation}
%\hassan{@Ben, I think it will be useful to argue here why we think NER models like spaCy might be available as a service? Are there some existing examples out there? We can also motivate the use of passwords as an example. Like the fact that there may be a dictionary available, so the search space is not infinite. Recall that membership inference requires that we know the exact target data point}
%\ben{added section}

The volume of intellectual property generated by small, medium and large enterprises is increasing at a growing rate, as reflected by sustained growth in the document management services industry~\cite{docu_manage_FBI_2020}. Particularly in industries like finance~\cite{SEC_finance_retention} and Health sector~\cite{AHIMA_med_retention}, where regulations dictate records be held for a minimum amount of time. Coupled with a sense of cyber-awareness, companies may seek to sanitize their documents, removing any sensitive information that may incur regulatory retaliation, or disruption to business in the event of a breach. However, with such volume of data, it increasingly drains human resources to sort and redact sensitive information. This is where automated text redaction services are appealing, with the opportunity to process sensitive documents at scale. We have begun to observe innovation in the space of text redaction from the traditional rule based systems~\cite{pearl2016data,ibm_redact} to the use of AI-based systems~\cite{csi_intellidact,mphasis_airedact,aws_airedact}, particularly NER, in pursuit for higher accuracy and robustness to multiple manifestations of sensitive information. The appeal of NER is allowing companies to personalize the model for their own use case.

This personalization, on the flip side, has the potential for unintended memorization of the training examples as previously reported for neural networks in general~\cite{shokri2017membership}.
This memorization is particularly true when dealing with data that is not considered ``standard'' personal identifiable information (PII), like passwords. Passwords may be communicated and/or recorded in technical documentation. Due to their sensitive nature, there is a desire to redact this information.

Consider the scenario whereby a document management company adds an additional entity for recognition and redaction using labelled data they have on hand, including these passwords. The company would have had obtained and labeled documents, to update a base model provided as a pre-trained model in an offline or online setting to ensure compatibility with their system.

This updated NER model may then be provided as a service to complement their core business of document management. This can be done by providing API access to the NER model for their customers to perform text redaction query by query, or to interface directly with their customer systems. An attacker with access to the same API may be able to infer the passwords used to train the updated NER model (for the updated entities), via a membership inference attack~\cite{shokri2017membership,yeom2018privacy,salem2019ml,zhao2021feasibility}. The attacker with possession of a dictionary of candidate passwords may be able to infer which passwords were used to update the NER model if it is susceptible to membership inference attacks. 

%of a set of possible passwords, may be feasible, as a dictionary of candidate passwords can be obtained from previously leaked passwords. This substantially reduces the search space of passwords to attainable levels.


% \hassan{I think we probably do not need to talk about attribute inference. May be more a case for why the updated NER model would be allowed to be used as a service? We can of course assume that the attacker can launch a membership inference attack in the sense that the attacker would have a dictionary of passwords.} 
% \blue{Consider the scenario whereby a company seeks to profit from an updated NER model, or a company providing a NER model as a service to complement their core business of document management. In such a setting, the company would need to obtain and label documents, to update a base model provided as a pre-trained model in an offline or online setting to ensure compatibility with their complementary offerings. This company may provide API access to the NER model for their customers to perform text redaction query by query, or to interface directly with their customer systems.}
% We acknowledge that recovering an entire password from scratch is an inherently difficult task, akin to Attribute Inference~\cite{yeom2018privacy,zhao2021feasibility}. However, the simpler task of Membership Inference~\cite{shokri2017membership,yeom2018privacy,salem2019ml,zhao2021feasibility}, which requires possession of a set of possible passwords, may be feasible, as a dictionary of candidate passwords can be obtained from previously leaked passwords. This substantially reduces the search space of passwords to attainable levels.

==> MI-text classification - PETS 2023/timing_side_channel.tex <==
\section{Membership Inference via Timing Attack}\label{sec:MIA_timing}
In this section, we propose a timing side-channel attack on NER models from observations that models process traning dataset words faster. The attack in prior sections was specific to memorization in the NN model, this attack targets the tokenizer which internally accesses a vocabulary maintained by the NER pipeline.
Like that of Section~\ref{threat_model}, the updated NER model is available to the attacker via black-box access, with an attacker objective to infer membership of sensitive training data used to update the model. An important distinction of this MI attack, is that surrounding sentences are inessential, and thus knowledge of the surrounding sentence is not assumed. 

\subsection{Timing attack methodology}
% \footnote{https://spacy.io/models/en}

\subsubsection{Vocabulary}
A pretrained NER pipeline contains many components (We specifically evaluate spaCy's pre-trained \newline ``en\_core\_web\_lg'' and  ``en\_core\_web\_trf'' pipeline~\cite{spacy}, the key difference being the tokenizer, of which ``tok2vec'' and a ``ROBERTA based transformer'' is used respectively), each component can be treated as a separate model to be updated with user data. 
%
In these pipelines, there exists a vocabulary containing word associated strings (prefix, suffix, shape and norm) of the pre-training dataset. We call this the \textit{original vocabulary}. When one updates the pipeline with their private dataset, the vocabulary of the pipeline is updated with strings (prefix, suffix, shape and norm/lowercase for tok2vec, and byte-level byte pair encodings for the ROBERTA-base transformer) from the updating dataset (The \textit{updated vocabulary}), becoming a superset of the original vocabulary. Words within a vocabulary are in-vocab words, and those not are out-vocab words.

\subsubsection{Intuition Behind the Attack} 
The exploit occurs when the model takes additional time processing out-vocab words. Specifically, when a word passes through the pipeline, the tokenizer first extracts the tokens of the word which are checked in the vocabulary. If present, nothing changes, if not present, they are added to the vocabulary. Thus, vocabulary updates on new out-vocab words are likely to take longer. 
%
% We remark that the timing difference persists even if two different words have the same set of features. SpaCy still adds new words even with similar features with an existing word in the vocabulary. An example is shown in Appendix~\ref{app:equiv-proof}.
%
Member words from the training/update set are already present in the vocabulary, in contrast to unseen non-member words. This, presents an opportunity for an attacker to infer membership based on the inference time. 

For this attack, position ourselves as a black box attacker, leveraging only the execution time from the time of query to the time the output is returned. The assigned label and confidence of the word is ignored (Though there remains a potential to fuse these features). We demonstrate this attack with a password use-case, with an updated NER model is specifically trained to label passwords in documents. Again, the adversary's goal is to infer membership of passwords used in the updating (private) dataset. 


\subsubsection{Attack on the Original NER Model}
\label{subsec:attack_orig_ner}
We first evaluate the timing side-channel attack on two public spaCy NER models. 
%
By accessing the pretrained vocabulary strings, we can establish the ground truth for members, or \textit{in-vocab set}. We remark that in practice, a black box attacker would not have simple access to the model vocabulary. Next, we generate a set of out-vocab words such that at minimum their `suffix' and `shape' are not in the original vocabulary's string table (the same set is used to evaluate the transformer pipeline). We note that we exclude the prefix feature when generating out-vocab words due to unavoidable overlaps with in-vocab words (by default, the first character of the word). 
Specifically, we generate a list of 5000 random passwords where each password has minimum length of 6 characters including at least 1 of each: uppercase, lowercase character, digit and special symbol. We refer to these generated passwords as the \textit{out-vocab set}.


\descr{Experimental Setup.} We randomly sample 2000 words from the \textit{in-vocab set} and 2000 password from the \textit{out-vocab set}. Then, we sequentially query the original NER model interleaving between in-vocab and out-vocab words. We alternate to ensure consistent delay across both sets as a result of other spurious processes on the system. Each query is simply a single word with no surrounding text, with a measurement of the time taken to process the query. 
From the execution time, the attacker can choose a threshold to classify the queried word as a member or non-member. For our evaluation we present the ROC curve and the AUC as a general measure of classification performance.

\subsubsection{Attack on an Updated NER Model}
\label{timing_attack_updated_ner}
We also evaluate an updated version of the NER model. Starting with the clean pretrained NER models, we update them with a subset of our generated passwords. 
To update the NER model, we generate 5000 passwords like Section~\ref{subsec:attack_orig_ner}, reserving the first 2000 passwords (\textit{updating dataset $D_u$}) to update the NER model. 
The NER model update includes teaching the NER to identify sensitive words with the new SECRET label. Specifically, training examples are in the form $s[r] = \text{``Alice's secret is $r$.''}$, where $r$ is a password from $D_u$, annotated as:
\begin{quote}
   ``Alice's secret is $r$.'',
\{`entities': [(0, 5, `PERSON'), (18, 18 + length($r$), `SECRET')]\}
\end{quote}
% With $\$word\$$ is replaced by the password in the dataset for updating the model.
%\hassan{<-- reconcile this with the updated notation: we have phrases $s[r]$}
% Specifically, the input samples to the updating process including the phrases and a new label \textit{SECRET}. 
% Hence, the updated NER model is now able to recognise 19 predefined named entities, i.e. The SECRET entity added to the 18 entities in the original model. %\hassan{The 18 named entities being part of the spaCy should also come earlier when we are introducing spaCy}

\descr{Experimental Setup.} We sample 2000 passwords from the remaining 3000 generated passwords. Then, we query the updated NER model with 2000 $r\in D_u$ (in-vocab) and 2000 $r\notin D_u$ (out-vocab), in an alternating manner. The execution time to output return for each query is measured. 
% The execution time to get an output for each updating password serve as the execution time the model needs to process a query about a member of the training (updating) dataset. In contrast, for a query about a generated password which the model has never seen will serve as the execution time the model needs to process a non-member of the training dataset. 
Again, the attacker can choose a threshold to classify the queried word as a member or non-member, though we present the ROC curve and the AUC as a general measure of performance.
% We use these two execution time sets as inputs to our attack's classifier. 

\subsection{Timing Attack Results}
% In our classifier \hassan{Once again it is not a classifier}, we specify member and non-member words as negative and positive class respectively. 
% Note that we perform our attack on original NER model by querying it with in-vocab words and out-vocab words. 

  
\descr{Timing Attack.} 
Figure~\ref{fig:timing_sid_channel} shows the receiver operating characteristic (ROC) curve and the AUC values of our attack on the original NER and the updated NER models.
We observe significant ease in inferring membership of words in both the original the updated NER pipelines. The lowest AUC is 0.9923, and is consistent across both the ``tok2vec'' and the ROBERTA based transformer pipelines. In both pipelines, the updated NER is marginally more susceptible to MI. It is clear that timing attacks against these pipelines are effective

We provide an expanded view of the in-vocab and out-vocab times in Figure~\ref{fig:absolute_time_ner} of Appendix~\ref{sec:app:timing}. From those figures, it can be observed in every setting, the NER model takes more time to process words that are outside the pre-trained vocabulary (in the original NER model) and outside of the updating dataset (in case of the updated NER model).





\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{plots/timing_attack_auc.pdf}
% \vspace{-2mm}
\caption{Timing side-channel attack ROC curve to classify membership of word inputs for the original pre-trained and updated NER model, on both tok2vec and transformer pipelines. {Note that the x-axis does not span to 1.}
}
\label{fig:timing_sid_channel}
% \vspace{-3mm}
\end{figure}

% \hassan{This is very thin. What happened to first, second and third run? The analysis should be much deeper}
% \hassan{Also, argue here why updating the model with larger text will not make any difference for the timing attack}

\descr{Querying Non-Members Multiple Times.}  
Following the attack we observe that the features of even non-member words will be added to the vocabulary of the model. Noting the fact that spaCy's NER pipeline will add features of any new word into the vocabulary, we continue our attack on both versions of the NER model where an adversary queries the model with the same word (in-vocab and out-vocab) two more times. Surprisingly, we still obtain AUCs of greater than 0.8195 for both models and pipelines with the execution time of the model to process words on its \textit{second} or \textit{third} query (In full, 0.820, 0.994, 0.994, 1.00, for 2nd run, and 0.995, 0.995, 0.993, 0.999 on the 3rd run for Original LG, Updated LG, Original TRF, and Updated TRF respectively). 
% This indicates that updating the vocabulary during the tokenization process is not the only vulnerability making the NER model prone to timing membership inference attacks.
{The persistence of timing vulnerability despite the vocabulary update means that there are additional components within the processing pipeline that are not updated, resulting in sufficient timing differences for successful membership inference. Regardless, we can conclude that NER models take more time to process words they are not trained on.} 

%\hassan{querying Non-Members Multiple Times: what is the reason of the increased inference time of testing samples beyond vocabulary update?
%We do not have a reason why multiple queries beyond the vocabulary update still offer sufficient timing differences for membership. We have highlighted this observation, though we shall add our hypothesis that of additional model components not updating in subsequent queries as the cause for timing discrepancy
%}

% We check the vocabulary of the updated NER model after performing our attack and observe that all features of non-member words have been added to the vocabulary. % once the model processed it. 
% Noting the fact that the spaCy pipeline for NER task will add features of any new word into the vocabulary, we continue our attack on both versions of the NER model where adversary queries the model with the same word (in-vocab and out-vocab) two more times. 
% Surprisingly, we still get AUCs of greater than 0.97 for both attacks when we use the execution time taken by the model to process the words on its \textit{second} or \textit{third} query. This exposes the fact that the NER model always takes more time to process words that it has never been trained on. This indicates that updating the vocabulary during the tokenization process is not the only vulnerable operation making the NER model prone to membership inference attack. 







==> MI-text classification - PETS 2023/todos.tex <==
\section{{\color{red}TODOS}}

{\color{red}
\begin{enumerate}
    \item Distance backed check of volcab words and passwords
    \item White box attack on volcab (additions to the table)
    \item Black box attack on side channels. (unseen words should take longer due to need to compute vectors).
    \item Password shape influence on ranks.
\end{enumerate}
}

{\color{red} Notes 18/02/21
\begin{enumerate}
    \item System level attack: black-box / white box
    \item Attacking the 'ner': memorization
    \item Black box on side channels: investigating when seeing new words: adding strings to the voacab.strings table, assigning the last vector in the pre-computed vector table to new words. 
    \item White box attack on the tokenizer: seeing the vocab.strings table before and after update the model; new words will get the same vector (from the last vector in the pre-computed vector table)
    \item Check the output layer: investigating the OUT label given to the word the probability given to the OUT-label word. Can be a hint for non member or member.
    \item Defense: potential defense to the model update (resume training); differential privacy; Side channel attacks: timer delays/constraints;
\end{enumerate}
}

==> MI-text classification - PETS 2023/usecases.tex <==
\section{Use Cases}
\paragraph{Document Redaction}
Considering a setting where text classification models are used to classify and redact sensitive information from a given document~\cite{song2019auditing}. If an adversary has black-box access to the model and the redacted document used for training, the adversary could use the model's text classification feature to identify if some text was in the training data that was redacted. As we demonstrate in our work, and as seen in previous works~\cite{nivre2004incrementality}, dependency parser models like Spacy~\cite{honnibal2015improved} could be used to redact sensitive information from text. These models are trained on sensitive information to be classified as per need, the probability scores assigned to words per class could inadvertently leak information of the sensitive data used for training the models.


\paragraph{Text Classification Models}

==> memorization_based_attack.tex <==
\section{Memorization}
Having introduced the privacy risks involved with text classification models used specifically for documents redaction tasks, we now describe the experimental methods used to evaluate the memorization and exposure of sensitive information which could further lead to uncover the redacted information of texts used for training of the model. We experiment with the pretrained language models provided by spaCy.

\subsection{Overview}

\subsection{Methodology}
\subsubsection{Memorization}
In our experiments, we use spaCy's NER component, which is a trainable component, so we are able to add new classes to the NER system and update the model with user defined examples. The examples that need to be fed to the model before training are required to be annotated by labeling words in the sentence to a corresponding label. 

We generated random phrases of a specific sequence format $s$ = ``Alice's secret is *****'' where the asterisks are replaced by a secret picked from a randomness space $r$. This method is build upon the existing work in \cite{carlini2019secret}, by  formally defining the sequence format with a secret information as $s[r]$ which refers that the asterisks are to be replaced from randomness space $r$. That inserted secret $\hat{r}$ is a word or number is randomly picked from the randomness space. For example, a secret could be a random password picked at random from a randomness space as big as a publicly available password dictionary and one such example could $s[\hat{r}]$ = ``Alice's secret is qwertyui''.

In our experimental methods:

\begin{enumerate}
    \item We test out memorization by doing a membership inference attack by first updating the model with a single phrase (e.g., ``Alice's secret is qwertyui'') that contains an out of distribution word (e.g., ``qwertyui'') picked randomly from a set of passwords and then querying the model with the whole set of password to see which password is given the highest probability score.
    % \item We use the rank metric described in Section \ref{evaluation_metrics} to rank the passwords based on exposure value, the higher the exposure, the more the model has that word memorized.
    \item We use the rank metric (Section \ref{evaluation_metrics}) based on the probability scores assigned to the password in the text to investigate how the memorized word ranks the highest each time.
    \item To get an average of the rank of the queried password, we run the same experiment on $N$ different passwords (e.g., training the model with 1 password at a time) and to average out for each password we train the model 48 times. The number is picked due to the strictness of resources.
    \item We tweek the experiments with multiple number of insertions and increasing the number of epochs to see at what point the model completely memorizes the trained sequence. The memorization is shown in figure \ref{fig:memorization-spacy}.
    \item We generate passwords to train the model with, using password strength \cite{wheeler2016zxcvbn} and investigate the level of memorization for different scores of strength.
    
\end{enumerate}

\subsubsection{Extraction}
To extract the password memorized by the model we propose to target the model's feature extraction layer where the model uses sub-word feature for each word queried to the model. For the extraction of the learned password:
\begin{enumerate}
    \item We analyze the effect of sub-word feature vectors that we have discussed in Section \ref{ner_spacy}. SpaCy uses multiple sub-word features while embedding the words into a context independent vector representation. 
    \item We use a \textit{feature distance metric} to see how passwords, who are close to the trained password rank higher than the password as they move away with respect to those features..
    \item Based on the features of the trained passwords, we generate similar passwords to analyze the impact of features with respect to the distance metrics and the rank.
    \item We formulate an algorithm to extract a password unknown to the adversary by querying the model taking into consideration one feature at a time and getting closer to the target password by finding the passwords with similar features.
    
\end{enumerate}
With the extraction strategy, even if the exact password is not recovered, some features of the password are extracted that reduces the search space of a brute force algorithms by a significant degree.


\subsection{Evaluation}
\subsubsection{Evaluation Metrics}
\label{evaluation_metrics}
In this section, we will define the metrics used to evaluate the extent of memorization and the privacy risk of sensitive information or an inserted secret in the training data of the model. We adapt the exposure metric from the secret sharer \cite{carlini2019secret} with slight modifications in context of our setting. Firstly, we define the rank of the inserted secret, this metrics is slight different to the work in \cite{carlini2019secret} as they used the perplexity scores provided by the model for a given text whereas in our case, we use the probability score assigned to the target class of the secret word/phrase.

Given a secret phrase i.e. $s[r]$ = ``Alice's secret is qwertyui", including some secret information ${r}$ sampled randomly from a randomness space $\mathcal{R}$. In this example, the secret is a password picked randomly from a list of $\mathcal{R}$ possible passwords from a password dictionary. The rank of the secret is defined as the index in the list of randomly picked $\mathcal{R}$ passwords, ordered by the probability scores assigned to each individual password $s[{r}]$, for a particular known class, in this case ``PASSWORD".
\\
\textbf{Metric 1} \textit{The rank of a secret $s$ is then defined as}
$$ \textbf{rank}(s[r]) = |\{r' \in \mathcal{R} :Pr(s[r']) \leq Pr(s[r])\}| $$
\\
Where $Pr(s[r])$ is the probability of the secret $r'$ in the phrase $s$ randomly picked from a randomness space $\mathcal{R}$ where it should be greater than all the other possible secrets $r'$ from the same randomness space.

\subsection{Experimental Results}
We experiment the memorization of out of distribution words on two different versions of spaCy. We see that both the versions memorize out of distribution words with high probability, however, the newer release of spaCy shows faster memorization as depicted in Figure \ref{fig:memorization-spacy}.

\begin{figure}
\centering
\begin{tabular}{c}
\subfloat[spaCy 2.3.2]{\includegraphics[width=\linewidth]{plots/SpaCy_2.3.2_RANK_PER_EPOCH_AND_INSERTION.png}}\label{fig:spacy2} \\
\subfloat[spaCy 3.0.3]{\includegraphics[width=\linewidth]{plots/spaCy3.0.3_RANK_PER_EPOCH_AND_INSERTION.png}} \label{fig:spacy3}
\end{tabular}
\caption{The extent of model memorization for out-of-distribution words in two different versions of spaCy. ``Insertions'' refer to the number of times the same phrase is repeated in the training set, ``Epochs'' is the number of training iterations the model undergoes during the update process. ``Ranks'' is calculated using the exposure metric based on the probability score assigned to the label.}
\label{fig:memorization-spacy}
\end{figure}



==> motivation.tex <==
\section{Motivation}
Previously, the redaction of sensitive information from documents is a highly manual task requiring expertise and many hours to complete~\cite{gordon2013mra}. One of the major problems with redaction is that it can't be always content based, and for redacted information based on context more sophisticated process are required and as more documents are being generated, proposals have been made to Automate document redaction to provide cost and time savings for the privacy-conscious document holder using text classification algorithms in natural language processing; However with the use of machine learning techniques for effective text classification, and subsequently text redaction may lead to privacy risks for the data used to train the models. To identify sensitive information, sensitive information would be used to train models, particularly if a model is to be tailored for a specific set of policies, a personalized process for each different company. NER system has been used to identity sensitive information in various settings~\cite{gomez2010data, ge2020fedner, kanchana2020optical} and hence has pose a risk to the sensitivity of the data used during training.

It is because this personalized training of the model requires company data, we show in our initial experiments, that the update set used to train the model would be susceptible to membership inference attacks.

If the model is updated with a training set whereby the same piece of sensitive information occurs a significant number of times, the model is able to memorize the sensitive information. Consequently, leading to an attacker finding membership information, and even potentially recovering the sensitive information. 
It is very likely that such sensitive information repeats itself in the training set, for example user emails may be at risk, when redacting emails, with repeated emails, the model is repeatedly exposed to the sender's signature block which is very likely to include personal information of the sender.



==> old_abstract.tex <==
\begin{abstract}

Named entity recognition models (NER), also known as entity identification or entity extraction systems, are widely used for the tasks of identifying named entities (e.g. individuals, locations, drugs, clinical procedures, etc.) in text documents. Machine learning based NERs are often applied to privacy-sensitive applications that need automatic and scalable identification of sensitive information to de-identify personal information and to redact text for data sharing. \dali{add a note on how the training of these models is done? May be an example from the health/medical sector}\rana{We do talk about how the pretrained spacy model is updated with a collection of documents with new entities/labels.}



%\textbf{todo \dali{introduce NER and Machine learning based NERs. Then introduce applications of NER and the privacy perspective}}

%show great promise in many privacy-sensitive applications where they can automatically identify sensitive information in documents to protect against data breaches, to de-identify personal information, and to redact text for data sharing. These applications are inherently trained on sensitive datasets. 

In this paper, we study the case when an NER model is made available to end users as a black-box service identifying sensitive information in their documents and show that these models are vulnerable to attacks inferring information about their training datasets. 


Using the NER model from spaCy~\cite{spacy} \dali{did we use only one model from SpaCy?}\ben{Two versions of Spacy, same provider, slightly different architectures} as a representative implementation, a widely-used open-source natural language processing library, we demonstrate two attacks on these models. 

Our first attack is linked to the underlying neural network (NN) used in the NER model. It demonstrates how to exploit unintended memorization of NNs, a phenomenon NNs are known to be vulnerable to, in the context of NER to \dali{What's the attack objective? What did we demonstrate when exploiting the memorization? in a general sense, not findings specific.}\rana{memorization is exploited for text redaction applications and the ability to retrieve training data information having access to a redacted document used during training}.


Our second attack targets NER models that maintain vocabularies constructed from the training data 
\dali{Speedups of what?} \dali{Can we name these models? i.e. refer to them according to some widely used/accepted terminology...}. \ben{resolved, speedup removed, volcabulary is acccepted terminology}
We show that these models are vulnerable to timing attacks, exploiting the different execution paths taken by words in the training dataset in comparison to words that were never seen by the model. \dali{Same than attack 1. Can we say in a general sense what the attack aims to do. inferring membership in training sets, or some leakage from the training set?? } \ben{Both attacks seek to leak membership information about the training dataset, which in the context of passwords is a security risk, and in the health dataset, a privacy/regulation problem}

We experimentally demonstrate our attacks by updating the public spaCy NER model with phrases containing sensitive information. 

Our results show that the model memorises even when the update contains a single phrase. 

We also demonstrate a membership inference attack \dali{the wording membership inference attack is coming out of the blue here!} \ben{perhaps: We also demonstrate an inference attack to determine the membership of sensitive information contained within the training dataset.} on a document redaction use-case, resulting in more than 70\% AUC. We show that the timing attack is overwhelmingly successful with an AUC of 98.84\%. Finally we discuss some mitigation techniques which can be adopted to make NER models resilient against inference attacks \dali{"some" mitigation techniques is way too vague. I suggest you provide reasonable information about how to mitigate the attacks. If we didn't provide any experimental analysis of the defense techniques, best is to remove this last note}.\ben{we only speculate about defence mechanisms} \ben{perhaps: Finally we discuss potential mitigation approaches to realize the safe use of NER models in light of the presented privacy and security implications of membership inference attacks.}
\end{abstract}

==> todos.tex <==
\section{{\color{red}TODOS}}

{\color{red}
\begin{enumerate}
    \item Distance backed check of volcab words and passwords
    \item White box attack on volcab (additions to the table)
    \item Black box attack on side channels. (unseen words should take longer due to need to compute vectors).
    \item Password shape influence on ranks.
\end{enumerate}
}

{\color{red} Notes 18/02/21
\begin{enumerate}
    \item System level attack: black-box / white box
    \item Attacking the 'ner': memorization
    \item Black box on side channels: investigating when seeing new words: adding strings to the voacab.strings table, assigning the last vector in the pre-computed vector table to new words. 
    \item White box attack on the tokenizer: seeing the vocab.strings table before and after update the model; new words will get the same vector (from the last vector in the pre-computed vector table)
    \item Check the output layer: investigating the OUT label given to the word the probability given to the OUT-label word. Can be a hint for non member or member.
    \item Defense: potential defense to the model update (resume training); differential privacy; Side channel attacks: timer delays/constraints;
\end{enumerate}
}

==> usecases.tex <==
\section{Use Cases}
\paragraph{Document Redaction}
Considering a setting where text classification models are used to classify and redact sensitive information from a given document~\cite{song2019auditing}. If an adversary has black-box access to the model and the redacted document used for training, the adversary could use the model's text classification feature to identify if some text was in the training data that was redacted. As we demonstrate in our work, and as seen in previous works~\cite{nivre2004incrementality}, dependency parser models like Spacy~\cite{honnibal2015improved} could be used to redact sensitive information from text. These models are trained on sensitive information to be classified as per need, the probability scores assigned to words per class could inadvertently leak information of the sensitive data used for training the models.


\paragraph{Text Classification Models}
